The Role of Environment Access in Agnostic Reinforcement Learning

We study Reinforcement Learning (RL) in environments with large state spaces, where function approximation is required for sample-efficient learning. Departing from a long history of prior work, we consider the weakest possible form of function approximation, called agnostic policy learning, where the learner seeks to find the best policy in a given class $\Pi$, with no guarantee that $\Pi$ contains an optimal policy for the underlying task. Although it is known that sample-efficient agnostic policy learning is not possible in the standard online RL setting without further assumptions, we investigate the extent to which this can be overcome with stronger forms of access to the environment. Specifically, we show that: 1. Agnostic policy learning remains statistically intractable when given access to a local simulator, from which one can reset to any previously seen state. This result holds even when the policy class is realizable, and stands in contrast to a positive result of [MFR24] showing that value-based learning under realizability is tractable with local simulator access. 2. Agnostic policy learning remains statistically intractable when given online access to a reset distribution with good coverage properties over the state space (the so-called $\mu$-reset setting). We also study stronger forms of function approximation for policy learning, showing that PSDP [BKSN03] and CPI [KL02] provably fail in the absence of policy completeness. 3. On a positive note, agnostic policy learning is statistically tractable for Block MDPs with access to both of the above reset models. We establish this via a new algorithm that carefully constructs a policy emulator: a tabular MDP with a small state space that approximates the value functions of all policies $\pi \in \Pi$. These values are approximated without any explicit value function class.

==> sections/upper-bound-proofs-conc-version.tex <==
\clearpage
\section{Proof Attempt with Concentrability}\label{app:main-upper-bound}
\glcomment{copied this section over so that I could make changes which prove the concentrability version.}

In this section, we prove \pref{thm:conc-bmdp-result}.
\begin{assumption}[Factorized Concentrability]\label{ass:exploratory-conc-distribution}
    The exploratory distributions $\mu = \crl{\mu_h}_{h\in[H]}$ can be written as $\mu_h = \emission \circ \nu_h$ where $\nu_h \in \Delta(\cS_h)$ satisfies concentrability of the latent transitions.
\end{assumption}

\begin{theorem}\label{thm:conc-bmdp-result}
Under \pref{ass:exploratory-conc-distribution}, with probability at least $1-\delta$,
    \stochalg{} (\pref{alg:stochastic-bmdp-solver-v2})  returns an $\eps$-optimal policy using
    \begin{align*}
        \poly\prn*{ \cpush, S, A, H, 1/\eps, \log \abs{\Pi}, \log 1/\delta} \quad \text{samples.}
    \end{align*}
\end{theorem}
    
\subsection{Preliminaries}\label{app:upper-bound-preliminaries}
We will define some additional conceptions and notation which will be used in the analysis.

\begin{itemize}
    \item For any set $\cX' \subseteq \cX$ we denote the represented states as $\cS[\cX'] \coloneqq \crl{\optdec(x): x \in \cX'}$. For any $s \in \cS$ and subset $\cX' \subseteq \cX$ we let $n_s[\cX'] \coloneqq \abs{\crl{x \in \cX': \optdec(x) = s}}$ count the total number of observations there are emitted from a given state.
    \item We define the set of $\eps$-reachable latent states as
    \begin{align*}
        \epsRS{h} \coloneqq \crl*{s_h: \max_{\pi \in \Pi} d^\pi_h(s) \ge \eps }.
    \end{align*}
    \gledit{
    \item We define the set of $\eps$-pushforward-reachable latent states from $(s,a)$ as 
    \begin{align*}
        \epsPRS{}(s,a) \coloneqq \crl*{s': \optlatp(s_h~|~ s_{h-1}, a_{h-1}) \ge \eps},
    \end{align*}
    Observe that if $s \in \epsRS{}$ then every state in $\epsRS{}(s,a)$ is $\eps^2/S^2$-reachable.
    \item Given $(s,a)$, for any $\cX' \subseteq \cX$, we let $\nrch[\cX'~|~s,a] \coloneqq \abs{\crl{x \in \cX': \optdec(x) = \epsPRS{}(s,a)}}$ and $\nurch[\cX'~|~s,a] = \abs{\cX'} - \nrch[\cX'~|~s,a]$.}
    \item \glcomment{older definitions which we might not need anymore.} We define the set of $\eps$-pushforward-reachable latent states
    \begin{align*}
        \epsPRS{h} \coloneqq \crl*{s_h: \max_{s_{h-1}, a_{h-1}} \optlatp(s_h~|~ s_{h-1}, a_{h-1}) \ge \frac{\eps}{S} },
    \end{align*}
    and furthermore let $\epsPRS{} \coloneqq \cup_{h=1}^H \epsPRS{h}$.
    \item For any $\cX' \subseteq \cX$, we let $\nrch[\cX'] \coloneqq \abs{\crl{x \in \cX': \optdec(x) = \epsPRS{}}}$ and $\nurch[\cX'] = \abs{\cX'} - \nrch[\cX']$.
\end{itemize}


\paragraph{Estimated Transitions and Projected Measures.} Recall that the ground truth latent transition is denoted $\optlatp: \latentsp \times \actionsp \to \Delta(\latentsp)$. We will use $\samplelatp$ to denote the empirical version of the latent transition which is sampled in \pref{line:sample-decode-dataset} of \pref{alg:stochastic-decoder-v2}:
\begin{align*}
    \samplelatp(\cdot ~|~ \optdec(x_{h-1}), a_{h-1}) = \frac{1}{\ndec} \sum_{x \in \cD} \delta_{\optdec(x)}.
\end{align*}
In addition, we introduce a notion of projected measures which will be used to relate the ground truth transition $P = \emission \circ \optlatp$ with the estimated transition $\estp$ of the policy emulator.
\begin{definition} \glcomment{made changes to define the support of the projected measure to be states which are $\eps/S$ reachable} \gledit{Fix a tuple $(s,a)$.} For a distribution $p \in \Delta(\cS)$, define the \emph{projected measure} onto the observation set $\bar{\cX} \subseteq \statesp$ as
\begin{align*}
    \projm{\bar{\cX}}(p) \coloneqq \sum_{s' \in \epsPRS{}(s,a)} p (s') \cdot \unif (\crl{\empobs \in \bar{\cX}: \optdec(\empobs_h) = s'}).
\end{align*}
Specifically, for any $\empobs \in \bar{\cX}$ we have:
\begin{align*}
    \projm{\bar{\cX}}(p)(\empobs) = p (\optdec(\empobs)) \cdot \frac{\ind{\optdec(\empobs) \in \epsPRS{}(s,a)}}{n_{\optdec(\empobs)}[\bar{\cX}]}.
\end{align*}
Furthermore, for any subset $\bar{\cX}' \subseteq \bar{\cX}$ we denote $\projm{\bar{\cX}}(p)(\bar{\cX}') = \sum_{\empobs \in \bar{\cX}'} \projm{\bar{\cX}}(p)(\empobs)$.
\end{definition}
Formally, $\projm{\bar{\cX}}$ is not a true probability distribution, as the total measure might not sum up to 1, as would happen if $p(s) > 0$ for $s \in (\epsPRS{}(s,a))^c$.

\paragraph{Test Policy Validity.}
In our analysis, we will modify \pref{def:valid-test-policy-dd} as below.
\begin{definition}[Valid Test Policy]
For a layer $h \in [H]$, we say a collection of policies $\Pitest_{h} = \crl*{\pi_{\empobs, \empobs'}}_{\empobs, \empobs' \in \estmdpobsspace{h}}$
    is a $\tau$-\emph{valid test policy set} for policy emulator $\wh{M}$ if the following hold.
    \begin{itemize}
        \item (Maximally distinguishing): $\pi_{\empobs, \empobs'} = \argmax_{\pi \in \cA \circ \Pi_{h+1:H}} \abs*{\wh{V}^\pi(\empobs) - \wh{V}^\pi(\empobs')}$.
        \item (Accurate): For all $\empobs, \empobs' \in \estmdpobsspace{h}$:
        \begin{align*}
            \abs*{V^{\pi_{\empobs, \empobs'}}(\empobs) - \wh{V}^{\pi_{\empobs, \empobs'}}(\empobs)} &\le \tau \quad \text{and} \quad    \abs*{V^{\pi_{\empobs, \empobs'}}(\empobs') - \wh{V}^{\pi_{\empobs, \empobs'}}(\empobs')} \le \tau.
        \end{align*}
    \end{itemize}
\end{definition}


\subsection{Supporting Technical Lemmas for Sampling}

In this section, we establish several technical lemmas which show that various conditions that we need in the analysis hold with high probability under samples from $M$.

\paragraph{Properties of Policy Emulator Initialization.} We prove several properties that hold with high probability when the policy emulator is initialized in \pref{line:init-start}-\ref{line:init-end} of \pref{alg:stochastic-bmdp-solver-v2}.

\begin{lemma}[Sampling of Pushforward-Reachable States]\label{lem:sampling-states} \glcomment{changed $\epsPRS{} \to \epsRS{}$.}
With probability at least $1-\delta$:
\begin{align*}
    \forall~ h \in [H], \forall~ s \in 
\epsRS{h}: \quad n_{s}[\estmdpobsspace{h}] \ge \frac{\eps}{2 \cconc S}\cdot \nreset.
\end{align*}
\end{lemma}

\begin{proof}
Fix any $s \in \epsRS{h}$. Let $Z^{(i)}$ be the indicator variable of whether observation $x^{(i)}_h \sim \mu_h$ satisfies $\optdec(x^{(i)}_h) = s$. We know that $\En[Z^{(i)}] \ge \eps/(\cconc S)$. By Chernoff bounds we have
\begin{align*}
    \Pr \brk*{ \frac{1}{\nreset} \sum_{i=1}^{\nreset} Z^{(i)} \le \frac{1}{2} \cdot \frac{\eps}{\cconc S}} \le \exp \prn*{-\frac{\nreset \cdot \eps}{8\cconc S}},
\end{align*}
so as long as
\begin{align*}
    \nreset \ge \frac{8\cconc SH}{\eps} \log \frac{S}{\delta},
\end{align*}
by union bound, the conclusion of the lemma holds.
\end{proof}

\begin{lemma}[Pushforward Policy Concentration over $\mu$]\label{lem:pushforward-concentration} \glcomment{we might actually need this for $\eps^2$-reachable states, but come back to this later.} Suppose that the conclusion of \pref{lem:sampling-states} holds. Then with probability at least $1-\delta$:
\begin{align*}
    \forall~ h \in [H], \forall~ (s, a) \in \epsRS{h} \times \cA: \quad 
    \max_{\pi \in \Pi}~\abs*{ \brk*{\pi \push \emission(s)}(a) - \brk*{\pi \push \unif(\crl{\empobs \in \estmdpobsspace{h}: \optdec(\empobs) = s})}(a) } \le \frac{\eps}{A}.
\end{align*}
\end{lemma}

\begin{proof}
Fix any $(s, a) \in \epsRS{h} \times \cA$. Also fix any policy $\pi \in \Pi$. Denote the set $\cX_{s} = \crl{\empobs \in \estmdpobsspace{h}: \optdec(\empobs) = s}$, and observe that $\cX_{s}$ is drawn i.i.d.~from the emission distribution $\emission(s)$. By Hoeffding bounds we have
\begin{align*}
    \Pr\brk*{ \abs*{\brk*{\pi \push \emission(s)}(a) - \brk*{\pi \push \unif(\crl{\empobs \in \estmdpobsspace{h}: \optdec(\empobs) = s})}(a)} \ge \frac{\eps}{A}} &\le 2\exp \prn*{ -\frac{2 n_{s}[\estmdpobsspace{h}] \eps^2}{A^2} } \\
    &\le  2\exp \prn*{ -\frac{\nreset \eps^3}{\cconc S A^2} }, &\text{(\pref{lem:sampling-states})}
\end{align*}
Applying union bound we see that as long as 
\begin{align*}
    \nreset \ge \frac{\cconc SA^2}{\eps^3} \cdot \log \frac{2SAH\abs{\Pi}}{\delta}
\end{align*}
the conclusion of the lemma holds.
\end{proof}

\begin{lemma}[Sampling Rewards]\label{lem:sampling-rewards}
With probability at least $1-\delta$, every reward estimate $\wh{R}(\empobs,a)$ computed in  \pref{line:reward-estimation} of \pref{alg:stochastic-bmdp-solver-v2} satisfies $\abs{\wh{R}(\empobs, a) - R(\empobs,a)} \le \eps/H$.
\end{lemma} 
\begin{proof}
This follows by Hoeffding inequality and union bound over all $\nreset\cdot AH$ pairs $(\empobs, a) \in \estmdpobsspace{} \times \cA$.
\end{proof}

\paragraph{Properties of \stochdecoder{}.} Now we turn to analyzing a single call to \stochdecoder{}.

\begin{lemma}[Sampling Transitions]\label{lem:sampling-transitions} Fix any $(x_{h-1}, a_{h-1})$ for which we call $\stochdecoder{}$.  With probability at least $1-\delta$, the dataset $\cD$ sampled in \pref{line:sample-decode-dataset} of \pref{alg:stochastic-decoder-v2} satisfies
\begin{align*}
    \nrm*{\optlatp(\cdot~|~x_{h-1}, a_{h-1}) - \samplelatp(\cdot~|~x_{h-1}, a_{h-1})}_1 \le \eps.
\end{align*}
\end{lemma}
\begin{proof}
Every time a dataset $\cD$ is sampled, by concentration of discrete distributions we have for any $t > 0$:
\begin{align*}
    \Pr\brk*{\nrm*{\optlatp(\cdot~|~x_{h-1}, a_{h-1}) - \samplelatp(\cdot~|~x_{h-1}, a_{h-1})}_1 \ge \sqrt{S} \cdot \prn*{\frac{1}{\sqrt{\ndec}} + t}} \le \exp(-\ndec t^2).
\end{align*}
Setting the RHS to $\delta$ we have that with probability at least $1-\delta$, %
\begin{align*}
    \nrm*{\optlatp(\cdot~|~x_{h-1}, a_{h-1}) - \samplelatp(\cdot~|~x_{h-1}, a_{h-1})}_1 \le \sqrt{\frac{S \log (1/\delta)}{\ndec}}. 
\end{align*}
Therefore as long as 
\begin{align*}
    \ndec \ge \frac{S}{\eps^2} \cdot \log \frac{1}{\delta},
\end{align*}
the conclusion of the lemma holds.
\end{proof}

\begin{corollary}\label{corr:sampling-transitions} If the conclusion of \pref{lem:sampling-transitions} holds, then the proportion of observations from \gledit{$(\epsPRS{h}(x_{h-1}, a_{h-1}))^c$} in $\cD$ is at most $2\eps$.
\end{corollary}

\begin{lemma}[Pushforward Policy Concentration over Transitions]\label{lem:pushforward-concentration-transition}
Fix any $(x_{h-1}, a_{h-1})$ for which we call $\stochdecoder{}$. With probability at least $1-\delta$, the dataset $\cD$ sampled in \pref{line:sample-decode-dataset} of \pref{alg:stochastic-decoder-v2} satisfies
\begin{align*}
    \forall~ s \in \cS[\cD], \forall~a \in \cA, \forall~ \pi \in \Pi:\quad 
    \abs*{ \brk*{\pi \push \emission(s)}(a) - \brk*{\pi \push \unif\prn*{\crl*{ \empobs \in \cD: \optdec(\empobs) = s } } }(a) } \le \sqrt{\frac{2\log (2 SA \abs{\Pi}/\delta)}{n_s[\cD]}}.
\end{align*}
\end{lemma}

\begin{proof}
Fix a particular $s \in \latentsp[\cD]$, $a \in \cA$, and $\pi \in \Pi$. The set $\crl{\empobs \in \estmdpobsspace{h}: \optdec(\empobs) = s}$ is drawn i.i.d.~from the emission distribution $\emission(s)$. By Hoeffding bounds we have for any $t > 0$:
\begin{align*}
    \Pr\brk*{ \abs*{\brk*{\pi \push \emission(s)}(a) - \brk*{\pi \push \unif\prn*{\crl*{ \empobs \in \cD: \optdec(\empobs) = s } } }(a)} \ge t} &\le 2\exp \prn*{ -2 n_{s}[\cD] t^2}.
\end{align*}
By union bound over all $(s,a)$ and $\pi$, with probability at least $1-\delta$:
\begin{align*}
    \abs*{\brk*{\pi \push \emission(s)}(a) - \brk*{\pi \push \unif\prn*{\crl*{ \empobs \in \cD: \optdec(\empobs) = s } } }(a)} &\le \sqrt{\frac{2\log (2 SA \abs{\Pi}/\delta)}{n_s[\cD]}}
\end{align*}
This concludes the proof of the lemma.
\end{proof}

\begin{lemma}[Monte Carlo Estimates for \stochdecoder]\label{lem:monte-carlo}
Fix any $(x_{h-1}, a_{h-1})$ for which we call $\stochdecoder{}$. With probability at least $1-\delta$, every Monte Carlo estimate $\vest(\pi; x)$ computed in \pref{line:monte-carlo} of \pref{alg:stochastic-decoder-v2} satisfies
$\abs*{\vest(\pi; x) - V^{\pi}(x)} \le \eps$.
\end{lemma}

\begin{proof}
By Hoeffding's inequality we know that for a fixed $(x, \pi)$ pair:
\begin{align*}
    \Pr\brk*{\abs*{\vest(\pi; x) - V^{\pi}(x)} \ge \eps} \le 2 \exp(-2\nmc \eps^2).
\end{align*}
In total, we call \pref{line:monte-carlo} at most $\abs{\estmdpobsspace{h}}^2 \le \nreset^2$ times. Therefore, by union bound, as long as 
\begin{align*}
    \nmc \ge K \cdot \frac{1}{\eps^2} \cdot \log \frac{\cconc SAH \abs{\Pi}}{\eps \delta }
\end{align*}
where $K>0$ is an absolute constant determined by the value of $\nreset$, then the result holds.
\end{proof}

\paragraph{Properties of \stochrefit{}.} Now we establish the accuracy of estimates in a single call to \stochrefit{}.

\begin{lemma}[Monte Carlo Estimates for \stochrefit]\label{lem:refit-monte-carlo-accuracy}
    With probability at least $1-\delta$, every Monte Carlo estimate computed by \stochrefit{} (\pref{line:mc1} and \ref{line:mc2} of \pref{alg:stochastic-refit-v2}) is accurate up to error $\eps$.
\end{lemma}

\begin{proof}
In \stochrefit{} we compute Monte Carlo estimates for $2\nreset^2 + 2\nreset^3 \cdot AH$ times, since there are $2\nreset^2$ possible certificates $(x, \pi)$ and for each one we perform Monte Carlo estimates over all of the $(\bar{x},\bar{a})$ pairs in our policy emulator $\estmdp$. By Hoeffding bound and union bound we see that as long as 
\begin{align*}
    \nmc \ge K \cdot \frac{1}{\eps^2} \cdot \log \frac{\cconc SAH \abs{\Pi}}{\eps \delta},
\end{align*}
for some absolute constant $K>0$, the conclusion of the lemma holds.
\end{proof}

\paragraph{Additional Notation.}
Henceforth, let us define several events:
\begin{itemize}
    \item $\eventemulator \coloneqq \crl*{\text{the conclusions of \pref{lem:sampling-states} --- \ref{lem:sampling-rewards} hold}}$. We have $\Pr[\eventemulator] \ge 1-3\delta$.
    \item $\eventdec_t \coloneqq \crl*{\text{the conclusions of \pref{lem:sampling-transitions} --- \ref{lem:monte-carlo} hold on the $t$-th call to \stochdecoder{}}}$. We have $\Pr[\eventdec_t ] \ge 1-3\delta$. Furthermore, define the random variable $T_\mathsf{D}$ to be the total number of times that \stochdecoder{} is called.
    \item $\eventref_t \coloneqq \crl*{\text{the conclusion of \pref{lem:refit-monte-carlo-accuracy} holds on the $t$-th call to \stochrefit{}}}$. We have $\Pr[\eventref_t ] \ge 1-\delta$. Furthermore, define the random variable $T_\mathsf{R}$ to be the total number of times that \stochrefit{} is called.
\end{itemize}
In the analysis, we will drop the subscript $t$ when referring to $\eventdec_t$ and $\eventref_t$ if clear from the context.


\subsection{Analysis of \stochdecoder}

This section is dedicated to establishing \pref{lem:main-induction}, which is the main inductive lemma.

\newcommand{\err}{\wh{\mathsf{Err}}}
Let us define the error term
\begin{align*}
    \err(s) \coloneqq \max_{x \in \estmdpobsspace{h}: \optdec(x) = s} \max_{\pi \in \Pi}~\abs*{V^\pi(x) - \wh{V}^\pi(x)}.
\end{align*}
The error term $\err$ is the worst case estimation error of $\estmdp$ for observations drawn from a latent state $s$.

\begin{lemma}[\glcomment{Attempt: Modified Induction for \stochdecoder}] Fix any layer $h \in [H]$. Assume that:
\begin{itemize}
    \item $\eventemulator$ and $\eventdec$ hold.
    \item \gledit{$\max_{\pi \in \Pi} \sum_{s' \in \latentsp_h} d^\pi_{h}(s') \cdot \err(s')  \le \Gamma_{h}$.}
    \item Input confidence set $\cP(x_{h-1}, a_{h-1})$ satisfies $\projm{\estmdpobsspace{h}}(\optlatp(\cdot ~|~ x_{h-1}, a_{h-1})) \in \cP(x_{h-1}, a_{h-1})$.
    \item $\Pitest_{h}$ are $\taudec$-valid test policies for the policy emulator $\estmdp$.
\end{itemize}

Then \stochdecoder{} returns confidence sets $\cP$ via Eq.~\eqref{eq:confidence-set-construction-v2} such that: 
    \begin{enumerate}
        \item[(1)] $\forall~ (x_{h-1}, a_{h-1}) \in \epsRS{h-1} \times \actionsp: ~\projm{\estmdpobsspace{h}}(\optlatp(\cdot ~|~ x_{h-1}, a_{h-1})) \in \cP$;
        \item[(2)] \gledit{$\forall~ \bar{p} \in \cP: \max_{\pi \in \Pi} \sum_{s \in \latentsp_{h-1}} d^\pi_{h-1}(s) \cdot \err(s)  \le \Gamma_{h} + \poly(S,A,H) \cdot \eps.$}
    \end{enumerate}   
\end{lemma}

\subsubsection{Structural Properties of the Decoder Graph}
For the lemmas in this section, we will assume the preconditions of \pref{lem:main-induction} and analyze properties of the decoder graph $\gobs$ constructed in a single call to \stochdecoder{}.

\begin{lemma}[Validity of Decoding Function]\label{lem:strong-validity-obs-decoding} Under the preconditions of \pref{lem:main-induction}, for every $x_l \in \cXL$, we have
\begin{align*}
    \crl{\empobs_r \in \cXR: \optdec(\empobs_r) = \optdec(x_l)} \subseteq \cT[x_l].
\end{align*}
\end{lemma}

\begin{proof}
The proof is a reprise of the argument used in Part (1) of \pref{lem:controlling-transition-error}. We prove this by contradiction. Suppose that there existed some $x_l \in \cXL$ and $\empobs_r \in \cXR$ such that $\optdec(x_l) = \optdec(\empobs_r)$ but $\empobs_r \notin \cT[x_l]$. Then $\empobs_r$ must have lost a test to some other $\empobs_r' \in \cXL$, i.e. there exists some $\empobs_r' \in \estmdpobsspace{h}$ such that
\begin{align*}
    \abs*{\vest(\pi_{\empobs_r, \empobs_r'};x_l) - \wh{V}^{\pi_{\empobs_r, \empobs_r'}}(\empobs_r) } \ge \taudec + 2\eps. \numberthis\label{eq:invalid}
\end{align*}
By accuracy of $\Pitest_{h}$, we have
\begin{align*}
    \abs*{ V^{\pi_{\empobs_r, \empobs_r'}}(x_l) - \wh{V}^{\pi_{\empobs_r, \empobs_r'}}(\empobs_r)} = \abs*{ V^{\pi_{\empobs_r, \empobs_r'}}(\empobs_r) - \wh{V}^{\pi_{\empobs_r, \empobs_r'}}(\empobs_r)} \le \taudec. \numberthis \label{eq:valid1}
\end{align*}
Furthermore, by \pref{lem:monte-carlo} we have 
\begin{align*}
    \abs*{ \vest(\pi_{\empobs_r, \empobs_r'};x_l) - V^{\pi_{\empobs_r, \empobs_r'}}(x_r) } = \abs*{ \vest(\pi_{\empobs_r, \empobs_r'};x_l) - V^{\pi_{\empobs_r, \empobs_r'}}(x_l) } \le \eps. \numberthis \label{eq:valid2}
\end{align*}
Combining \eqref{eq:valid1} and \eqref{eq:valid2} we get that
\begin{align*}
    \abs*{ \vest(\pi_{\empobs_r, \empobs_r'};x_l) - \wh{V}^{\pi_{\empobs_r, \empobs_r'}}(\empobs_r) } \le \taudec + \eps, 
\end{align*}
which contradicts \eqref{eq:invalid}. This proves the lemma.
\end{proof}

\begin{lemma}[Biclique Property]\label{lem:biclique}
Under the preconditions of \pref{lem:main-induction}, for any $s \in \cS[\cXL] \cap \cS[\cXR]$ the subgraph of $\gobs$ over vertices $\crl{x \in \cX_\mathsf{L} \cup \cX_\mathsf{R}: \optdec(x) = s}$ is a biclique.
\end{lemma}

\begin{proof}
Fix any $s \in \cS[\cXL] \cap \cS[\cXR]$. By \pref{lem:strong-validity-obs-decoding}, any $x_l \in \cXL$ such that $\optdec(x_l) = s$ has an edge to every observation $\crl{\empobs \in \cXR: \optdec(\empobs) = s}$ in $\gobs$. Therefore, the subgraph over $\crl{x \in \cX_\mathsf{L} \cup \cX_\mathsf{R}: \optdec(x) = s}$ forms a biclique in $\gobs$.
\end{proof}

\begin{lemma}\label{lem:eps-reachable-set-inclusion}
\gledit{Under the preconditions of \pref{lem:main-induction}, if $\bar{s} \in \epsRS{}$, for any connected component $\cc$:
\begin{align*}
    \epsPRS{}(\bar{s},a) \cap \cS[\ccL] \subseteq \epsRS{}(\bar{s},a) \cap \cS[\ccR].
\end{align*}}
\end{lemma}

\begin{proof}
Fix any $s \in \epsPRS{}(\bar{s},a) \cap \cS[\ccL]$. By \pref{lem:sampling-states}, since $s \in \epsPRS{}(\bar{s},a)$, there exist some $\empobs \in \cXR$ such that $\optdec(\empobs) = s$; in other words, $s \in \cS[\cXR]$. \glcomment{actually we need to use the fact that $s$ is $\eps^2/S^2$ reachable.} Furthermore by the biclique property (\pref{lem:biclique}) we know that all such observations $\empobs \in \ccR$. In particular this implies that $s \in \cS[\ccR]$, completing the proof.
\end{proof}

\begin{lemma}\label{lem:bound1}
Let $\empobs, \empobs' \in \cXR$ such that $\optdec(\empobs) = \optdec(\empobs')$. We have $\max_{a \in \cA, \pi \in \Pi}~\abs{ \wh{Q}^\pi(\empobs, a) - \wh{Q}^\pi(\empobs', a) } \le 2\taudec$.
\end{lemma}

\begin{proof}
Denote $\pi_{\empobs, \empobs'} = \argmax_{\pi \in \cA \circ \Pi} \abs{\wh{V}^\pi(\empobs) - \wh{V}^\pi(\empobs')}$ to be the test policy for the pair $\empobs, \empobs' \in \cXR$. By accuracy of the test policy we know that 
\begin{align*}
    \abs*{V^{\pi_{\empobs, \empobs'}}(\empobs) - \wh{V}^{\pi_{\empobs, \empobs'}}(\empobs)} &\le \taudec \quad \text{and} \quad    \abs*{V^{\pi_{\empobs, \empobs'}}(\empobs') - \wh{V}^{\pi_{\empobs, \empobs'}}(\empobs')} \le \taudec.
\end{align*}
Furthermore since $\empobs, \empobs'$ are observations emitted from the same latent state, $V^{\pi_{\empobs, \empobs'}}(\empobs) = V^{\pi_{\empobs, \empobs'}}(\empobs')$. Therefore
\begin{align*}
    \max_{a \in \cA, \pi \in \Pi} \abs*{\wh{Q}^\pi(\empobs,a) - \wh{Q}^\pi(\empobs',a)} &= \abs*{\wh{Q}^{\pi_{\empobs, \empobs'}}(\empobs, \pi_{\empobs, \empobs'}) - \wh{Q}^{\pi_{\empobs, \empobs'}}(\empobs', \pi_{\empobs, \empobs'})} \le 2\taudec.
\end{align*}
This concludes the proof of the lemma.
\end{proof}

\begin{lemma}\label{lem:bound2}
Fix any $x_l \in \cXL$. If $\empobs_r, \empobs_r' \in \cT[x_l]$, then $\max_{a \in \cA, \pi \in \Pi} \abs{\wh{Q}^{\pi}(\empobs_r, a) - \wh{Q}^{\pi}(\empobs_r', a)} \le 2\taudec + 4 \eps$.
\end{lemma}

\begin{proof}
By definition of $\cT[x_l]$ we have
\begin{align*}
    \abs*{\vest(\pi_{\empobs_r, \empobs_r'}; x_l) - \wh{V}^{\pi_{\empobs_r, \empobs_r'}}(\empobs_r) } \le \taudec+2\eps \quad\text{and}\quad \abs*{\vest(\pi_{\empobs_r, \empobs_r'}; x_l) - \wh{V}^{\pi_{\empobs_r, \empobs_r'}}(\empobs_r') } \le \taudec+2\eps.
\end{align*}
Using the fact that test policies are maximally distinguishing we have
    \begin{align*}
        \max_{a \in \cA, \pi \in \Pi} \abs*{\wh{Q}^{\pi}(\empobs_r, a) - \wh{Q}^{\pi}(\empobs_r', a)} = \abs*{\wh{V}^{\pi_{\empobs_r, \empobs_r'}}(\empobs_r) - \wh{V}^{\pi_{\empobs_r, \empobs_r'}}(\empobs_r')} \le 2\taudec + 4 \eps.
    \end{align*}
This proves the lemma.
\end{proof}

\begin{lemma}[Bounded Width of $\cc$]\label{lem:width-of-cc}
For any connected component $\cc \in \crl{\cc_1, \dots, \cc_k}$ in $\gobs$ we have 
\begin{align*}
    \max_{\empobs, \empobs' \in \ccR} \max_{a \in \cA, \pi \in \Pi} \abs{ \wh{Q}^\pi(\empobs, a) - \wh{Q}^\pi(\empobs', a) } \le 4S\taudec + 8S\eps.
\end{align*}
\end{lemma}

\begin{proof}
Let us take any $\empobs, \empobs' \in \ccR$. Since $\empobs, \empobs'$ belong to the same connected component, there exists a sequence of observations $\mathsf{seq} = (\empobs_1 = \empobs, \dots, \empobs_n = \empobs') \in \ccR^n$ such that for every consecutive pair $\empobs_i, \empobs_{i+1}$ there exists some $x_l \in \ccL$ such that $\empobs_i, \empobs_{i+1} \in \cT[x_l]$. 

Fix any $a \in \cA, \pi \in \Pi$. Now we will bound $\abs{ \wh{Q}^\pi(\empobs, a) - \wh{Q}^\pi(\empobs', a) }$. We will construct an auxiliar sequence  $\wt{\mathsf{seq}} = (\wt{\empobs}_1, \dots, \wt{\empobs}_k)$ for some $k \le n$ as follows:
\begin{itemize}
    \item Initialize $\wt{\mathsf{seq}} = \emptyset$.
    \item For $i = 1, \cdots n$:
    \begin{itemize}
        \item Add $\empobs_i$ to the end of $\wt{\mathsf{seq}}$.
        \item If there exists $\empobs_j$ with $j > i$ such that $\optdec(\empobs_i) = \optdec(\empobs_j)$ then set $i \gets j$.
    \end{itemize}
\end{itemize}
Observe that $\wt{\mathsf{seq}}$ satisfies the following conditions:
\begin{itemize}
    \item $\wt{\empobs}_1 = \empobs$ and $\wt{\empobs}_k = \empobs'$.
    \item  For every $s \in \cS$, at most two observations $\wt{\empobs} \in \mathrm{supp}(\emission(s)) \cap \ccR$ are found in $\wt{\mathsf{seq}}$, and these observations must appear sequentially.
    \item For any $i \in [k-1]$, if $\optdec(\wt{\empobs}_i) \ne \optdec(\wt{\empobs}_{i+1})$ then there exists some $x_l \in \ccL$ such that $\wt{\empobs}_i, \wt{\empobs}_{i+1} \in \cT[x_l]$.
\end{itemize}
Now we can apply triangle inequality to $\wt{\mathsf{seq}}$:
\begin{align*}
    \abs*{ \wh{Q}^\pi(\empobs, a) - \wh{Q}^\pi(\empobs', a) } \le \sum_{i=1}^k \abs*{ \wh{Q}^\pi(\wt{\empobs}_i, a) - \wh{Q}^\pi(\wt{\empobs}_{i+1}, a) } \le 4S\taudec + 8S\eps.
\end{align*}
The final bound relies on the aforementioned properties of $\wt{\mathsf{seq}}$ in conjunction with \pref{lem:bound1} and \pref{lem:bound2} to handle the individual terms in the summation. This completes the proof of \pref{lem:width-of-cc}.
\end{proof}

\subsubsection{Structural Properties of Projected Measures}
Now we will prove several lemmas regarding the projected measure of the empirical latent distribution
\begin{align*}
    \samplelatp = \frac{1}{\abs{\cXL}} \sum_{x \in \cXL} \delta_{\optdec(x)}.
\end{align*}
which is sampled in \pref{line:sample-decode-dataset} of a single call to \stochdecoder{}.



\begin{lemma}\label{lem:proj-cc-expression}
Under the preconditions of \pref{lem:main-induction}, for any connected component $\cc$ of $\gobs$ \gledit{which is generated by $(x_{h-1}, a_{h-1}) \in \epsRS{h-1} \times \actionsp$}:
    \begin{align*}
        \projR(\samplelatp)(\ccR) = \sum_{s \in \epsPRS{}(\cdot) \cap \cS[\ccL] \cap \cS[\ccR]} \samplelatp(s).
    \end{align*}
\end{lemma}

\begin{proof}\glcomment{in this proof we modified $\epsPRS{} \to \epsPRS{}(\cdot)$ shorthand.}
We compute that
\begin{align*}
    \projR(\samplelatp)(\ccR) &= \sum_{\empobs \in \ccR} \projR(\samplelatp)(\empobs) \\
    &= \sum_{\empobs \in \ccR} \frac{n_{\optdec(\empobs)}[\cXL]}{\abs{\cXL}} \cdot \frac{\ind{\optdec(\empobs) \in \epsPRS{} (\cdot) }}{n_{\optdec(\empobs)}[\cXR]}\\
    &= \sum_{ s \in \epsPRS{} (\cdot) } \frac{n_{s}[\cXL]}{\abs{\cXL}} \sum_{\empobs \in \ccR}  \frac{\ind{\optdec(\empobs) = s}}{n_{s}[\cXR]} \\
    &\overset{(i)}{=} \sum_{s \in \epsPRS{}(\cdot) \cap \cS[\ccR]} \frac{n_{s}[\cXL]}{\abs{\cXL}} \sum_{\empobs \in \ccR}  \frac{\ind{\optdec(\empobs) = s}}{n_{s}[\cXR]} \\
    &\overset{(ii)}{=}  \sum_{s \in \epsPRS{}(\cdot) \cap \cS[\cXL] \cap \cS[\ccR]} \frac{n_{s}[\cXL]}{\abs{\cXL}} \sum_{\empobs \in \ccR}  \frac{\ind{\optdec(\empobs) = s}}{n_{s}[\cXR]}.
\end{align*}
For $(i)$, observe that if $s \notin \cS[\ccR]$, then the sum $\sum_{\empobs \in \ccR}  \frac{\ind{\optdec(\empobs) = s}}{n_{s}[\cXR]} = 0$. For $(ii)$, we use the fact that $n_s[\cXL] = 0$ if $s \notin \cS[\cXL]$. From here, we apply the biclique lemma (\pref{lem:biclique}). The biclique lemma implies that if $s \in \cS[\ccR]$, then $\crl{x \in \cXL: \optdec(x) = s} \subseteq \ccL$, and therefore $\cS[\cXL] \cap \cS[\ccR] = \cS[\ccL] \cap \cS[\ccR]$. Furthermore for any $s \in \cS[\ccL] \cap \cS[\ccR]$, all of the observations $\crl{\empobs \in \cXR: \optdec(\empobs) = s} \subseteq \ccR$, so $n_s[\cXR] = n_s[\ccR]$. Thus we can continue the calculation as
\begin{align*}
    \projR(\samplelatp)(\ccR) &=  \sum_{s \in \epsPRS{}(\cdot) \cap \cS[\ccL] \cap \cS[\ccR]} \frac{n_{s}[\cXL]}{\abs{\cXL}} \sum_{\empobs \in \ccR}  \frac{\ind{\optdec(\empobs) = s}}{n_{s}[\cXR]}\\
    &= \sum_{s \in \epsPRS{}(\cdot) \cap \cS[\ccL] \cap \cS[\ccR]} \frac{n_{s}[\cXL]}{\abs{\cXL}} \sum_{\empobs \in \ccR}  \frac{\ind{\optdec(\empobs) = s}}{n_{s}[\ccR]} \\
    &= \sum_{s \in \epsPRS{}(\cdot) \cap \cS[\ccL] \cap \cS[\ccR]} \frac{n_{s}[\cXL]}{\abs{\cXL}} = \sum_{s \in \epsPRS{} \cap \cS[\ccL] \cap \cS[\ccR]} \samplelatp(s).
\end{align*} 
This concludes the proof of \pref{lem:proj-cc-expression}. \glcomment{did we use the fact that the states are in $\epsPRS{}$? seems like we didn't!}
\end{proof}

\begin{corollary}\label{corr:estimating-projR} Under the preconditions of \pref{lem:main-induction}, then
$\sum_{\cc \in \crl{\cc_j}} \prn{ \frac{\abs{\ccL}}{\abs{\cXL}} 
 - \projR(\samplelatp)(\ccR) } \in [0,2\eps]$ \gledit{which is generated by $(x_{h-1}, a_{h-1}) \in \epsRS{h-1} \times \actionsp$}.
\end{corollary}
\begin{proof}
For any $\cc$ we have
\begin{align*}
    \frac{\abs{\ccL}}{\abs{\cXL}} - \projR(\samplelatp)(\ccR) &= \frac{\abs{\ccL}}{\abs{\cXL}} - \sum_{s \in \epsPRS{}(\cdot) \cap \cS[\ccL] \cap \cS[\ccR]} \frac{n_{s}[\cXL]}{\abs{\cXL}} &\text{(\pref{lem:proj-cc-expression})} \\
    &= \frac{\abs{\ccL}}{\abs{\cXL}} - \sum_{s \in \epsPRS{}(\cdot) \cap \cS[\ccL]} \frac{n_{s}[\cXL]}{\abs{\cXL}} &\text{(\pref{lem:eps-reachable-set-inclusion})} \\
    &= \sum_{s \in \epsPRS{}(\cdot) \cap \cS[\ccL]} \frac{n_s[\ccL]}{\abs{\cXL}} + \sum_{s \in (\epsPRS{}(\cdot))^c \cap \cS[\ccL]} \frac{n_s[\ccL]}{\abs{\cXL}} - \sum_{s \in \epsPRS{}(\cdot) \cap \cS[\ccL]} \frac{n_{s}[\cXL]}{\abs{\cXL}}  \\
    &= \sum_{s \in (\epsPRS{}(\cdot))^c \cap \cS[\ccL]} \frac{n_s[\ccL]}{\abs{\cXL}}.
\end{align*}
The last equality uses the fact that by \pref{lem:eps-reachable-set-inclusion}, $s \in \epsPRS{}(\cdot) \cap \cS[\ccL] \Rightarrow s \in \cS[\ccR]$, so in particular by \pref{lem:biclique} we have $\crl{x\in \cXL: \optdec(x) = s} \subseteq \ccL$, so therefore $n_s[\cXL] = n_s[\ccL]$. 

Summing over all $\cc$ and applying \pref{corr:sampling-transitions} we get that
\begin{align*}
    \sum_{\cc \in \crl{\cc_j}} \frac{\abs{\ccL}}{\abs{\cXL}} - \projR(\samplelatp)(\ccR) = \sum_{\bbC \in \crl{\bbC_j}} \sum_{s \in (\epsPRS{}(\cdot))^c \cap \cS[\ccL]} \frac{n_s[\ccL]}{\abs{\cXL}} = \sum_{s \in (\epsPRS{}(\cdot))^c} \frac{n_s[\cXL]}{\abs{\cXL}} \in [0, 2\eps].
\end{align*}
This proves \pref{corr:estimating-projR}.
\end{proof}

\begin{lemma}\label{lem:relating-proj-to-empirical}
Under the preconditions of \pref{lem:main-induction}, for every $\pi \in \Pi$ and $\cc \in \crl{\cc_j}$ \gledit{which is generated by $(x_{h-1}, a_{h-1}) \in \epsRS{h-1} \times \actionsp$}: 
\begin{align*}
    \max_{a \in \cA}~\abs*{ \brk*{ \pi\push \projR(\samplelatp)(\cdot~|~\ccR)}(a) - \brk*{\pi \push \unif(\ccL)}(a) } \le \frac{\eps}{A} +  K \cdot \sqrt{\frac{S \log \tfrac{SA \abs{\Pi}}{\delta}}{\nrch[\ccL]}}  + \frac{\nurch[\ccL]}{\nrch[\ccL]},
\end{align*}
where $K>0$ is an absolute constant.
\end{lemma}
\begin{proof}
\glcomment{this proof should basically go through provided that we modify the definition of $\epsPRS{}$ as well as $\nrch$.}
Fix any $\pi \in \Pi$, $\cc \in \crl{\cc_j}$, and $a \in \cA$. We can calculate that: 
\begin{align*}
    \hspace{2em}&\hspace{-2em} \brk*{ \pi\push \projR(\samplelatp)(\cdot~|~\ccR)}(a) \\
    &= \sum_{\empobs \in \ccR} \frac{\projR(\samplelatp)(\empobs)}{\projR(\samplelatp)(\ccR)} \indd{\pi(\empobs) = a} \\
    &= \frac{1}{\projR(\samplelatp)(\ccR)} \sum_{\empobs \in \ccR} \frac{n_{\optdec(\empobs)}[\cXL]}{\abs{\cXL}} \cdot \frac{\ind{\optdec(\empobs) \in \epsPRS{}} \indd{\pi(\empobs) = a}}{n_{\optdec(\empobs)}[\cXR]} \\
    &= \frac{1}{\projR(\samplelatp)(\ccR)} \sum_{s \in \epsPRS{}} \prn*{ \frac{n_{s}[\cXL]}{\abs{\cXL}} \cdot \frac{1}{n_{s}[\cXR]} \cdot \sum_{\empobs \in \ccR}  \ind{\optdec(\empobs) =s} \indd{\pi(\empobs) = a} }\\
    &= \frac{1}{\projR(\samplelatp)(\ccR)} \sum_{s \in \epsPRS{} \cap \cS[\ccR] } \prn*{\frac{n_{s}[\cXL]}{\abs{\cXL}} \cdot \frac{1}{n_{s}[\cXR]} \cdot \sum_{\empobs \in \ccR}  \ind{\optdec(\empobs) =s} \indd{\pi(\empobs) = a} } \\
    &= \frac{1}{\projR(\samplelatp)(\ccR)} \sum_{s \in \epsPRS{} \cap \cS[\cXL] \cap \cS[\ccR] } \prn*{\frac{n_{s}[\cXL]}{\abs{\cXL}} \cdot \frac{1}{n_{s}[\cXR]} \cdot \sum_{\empobs \in \ccR}  \ind{\optdec(\empobs) =s} \indd{\pi(\empobs) = a} } \\
    &= \frac{1}{\projR(\samplelatp)(\ccR)} \sum_{s \in \epsPRS{} \cap \cS[\ccL] \cap \cS[\ccR] } \prn*{\frac{n_{s}[\ccL]}{\abs{\cXL}} \cdot \frac{1}{n_{s}[\ccR]} \cdot \sum_{\empobs \in \ccR}  \ind{\optdec(\empobs) =s} \indd{\pi(\empobs) = a} }.
\end{align*}
The last line uses the biclique lemma (\pref{lem:biclique}) in the same fashion as the proof of \pref{lem:proj-cc-expression}. Now we apply the conclusions of \pref{lem:pushforward-concentration} and \pref{lem:pushforward-concentration-transition}, along with the fact that for every $s \in \epsPRS{} \cap \cS[\ccL] \cap \cS[\ccR]$ we have $\crl{\empobs \in \cXR : \optdec(\empobs) = s } \subseteq \ccR$ as well as $\crl{\empobs \in \cXL : \optdec(\empobs) = s } \subseteq \ccL$ (which is again implied by the biclique lemma):
\begin{align*}
     &\brk*{ \pi\push \projR(\samplelatp)(\cdot~|~\ccR)}(a) \\
    \le\quad& \frac{1}{\projR(\samplelatp)(\ccR) } \sum_{s \in \epsPRS{} \cap \cS[\ccL] \cap \cS[\ccR] } \frac{n_{s}[\ccL]}{\abs{\cXL}} \cdot \prn*{ \brk*{\pi \push \emission(s)}(a) + \frac{\eps}{A} } \\
    \le\quad& \frac{1}{\projR(\samplelatp)(\ccR) } \sum_{s \in \epsPRS{} \cap \cS[\ccL] \cap \cS[\ccR] } \frac{n_{s}[\ccL]}{\abs{\cXL}} \cdot \prn*{\frac{\eps}{A} + \sqrt{\frac{2 \log \tfrac{2SA \abs{\Pi}}{\delta}}{n_s[\ccL]}} + \frac{1}{n_{s}[\ccL]} \cdot \sum_{\empobs \in \ccL}  \ind{\optdec(\empobs) =s} \indd{\pi(\empobs) = a}}\\
    =\quad& \frac{1}{\projR(\samplelatp)(\ccR) \abs{\cXL}} \sum_{ s \in \epsPRS{} \cap \cS[\ccL] \cap \cS[\ccR] } \prn*{ \frac{\eps}{A} \cdot n_{s}[\ccL] + \sqrt{2n_s[\ccL] \log \tfrac{2 SA \abs{\Pi}}{\delta}} + \sum_{\empobs \in \ccL}  \ind{\optdec(\empobs) =s} \indd{\pi(\empobs) = a} }
\end{align*}
By \pref{lem:proj-cc-expression}, we have $\abs{\cXL} \projR(\samplelatp)(\ccR) = \sum_{s \in \epsPRS{} \cap \cS[\ccL] \cap \cS[\ccR]} n_{s}[\cXL] = \nrch[\ccL] $. Using Cauchy-Schwarz we get that
\begin{flalign*}
\hspace{2em}&\hspace{-2em} \brk*{ \pi\push \projR(\samplelatp)(\cdot~|~\ccR)}(a) \\
    &\le \frac{\eps}{A} + K \cdot \sqrt{\frac{S \log \tfrac{SA \abs{\Pi}}{\delta}}{\nrch[\ccL]}} + \frac{1}{\nrch[\ccL]} \sum_{s \in \epsPRS{} \cap \cS[\ccL] \cap \cS[\ccR]  } \prn*{\sum_{\empobs \in \ccL}  \ind{\optdec(\empobs) =s} \indd{\pi(\empobs) = a} } 
    \\&= \frac{\eps}{A} + K \cdot \sqrt{\frac{S \log \tfrac{SA \abs{\Pi}}{\delta}}{\nrch[\ccL]}} + \frac{\abs{\ccL}}{\nrch[\ccL]} \cdot \frac{1}{\abs{\ccL}}  \sum_{s \in \epsPRS{} \cap \cS[\ccL] \cap \cS[\ccR]} \prn*{\sum_{\empobs \in \ccL}  \ind{\optdec(\empobs) =s} \indd{\pi(\empobs) = a} } \numberthis \label{eq:partial}
\end{flalign*}
Let us investigate the last term. We have
\begin{align*}
&
\frac{1}{\abs{\ccL}}  \sum_{s \in \epsPRS{} \cap \cS[\ccL] \cap \cS[\ccR]} \prn*{\sum_{\empobs \in \ccL}  \ind{\optdec(\empobs) =s} \indd{\pi(\empobs) = a} } \\
    =\quad& \frac{1}{\abs{\ccL}}  \sum_{s \in \epsPRS{} \cap \cS[\ccL]} \prn*{\sum_{\empobs \in \ccL}  \ind{\optdec(\empobs) =s} \indd{\pi(\empobs) = a} } &\hspace{-10em}\text{(\pref{lem:eps-reachable-set-inclusion})}\\
    \le\quad& \frac{1}{\abs{\ccL}}  \sum_{s \in \epsPRS{} \cap \cS[\ccL]} \prn*{\sum_{\empobs \in \ccL}  \ind{\optdec(\empobs) =s} \indd{\pi(\empobs) = a} } + \frac{1}{\abs{\ccL}}  \sum_{s \in (\epsPRS{})^c \cap \cS[\ccL]} \prn*{\sum_{\empobs \in \ccL}  \ind{\optdec(\empobs) =s} \indd{\pi(\empobs) = a} } \\
    =\quad& \brk*{\pi \push \unif(\ccL)}(a)
\end{align*}
Plugging this back into Eq.~\eqref{eq:partial} we get that
\begin{align*}
\brk*{ \pi\push \projR(\samplelatp)(\cdot~|~\ccR)}(a) &\le \frac{\eps}{A} +  K \cdot \sqrt{\frac{S \log \tfrac{SA \abs{\Pi}}{\delta}}{\nrch[\ccL]}} + \frac{\abs{\ccL}}{\nrch[\ccL]} \cdot \brk*{\pi \push \unif(\ccL)}(a),
\end{align*}
and rearranging and using the fact that $\brk*{\pi \push \unif(\ccL)}(a) \in [0,1]$ we get that
\begin{align*}
    \brk*{ \pi\push \projR(\samplelatp)(\cdot~|~\ccR)}(a) - \brk*{\pi \push \unif(\ccL)}(a) \le \frac{\eps}{A} +   K \cdot \sqrt{\frac{S \log \tfrac{SA \abs{\Pi}}{\delta}}{\nrch[\ccL]}}  + \frac{\nurch[\ccL]}{\nrch[\ccL]}.
\end{align*}
One can repeat the same steps to get the lower bound. Therefore,
\begin{align*}
    \abs*{ \brk*{ \pi\push \projR(\samplelatp)(\cdot~|~\ccR)}(a) - \brk*{\pi \push \unif(\ccL)}(a) } \le \frac{\eps}{A} +   K \cdot \sqrt{\frac{S \log \tfrac{SA \abs{\Pi}}{\delta}}{\nrch[\ccL]}} + \frac{\nurch[\ccL]}{\nrch[\ccL]}.
\end{align*}
This proves \pref{lem:relating-proj-to-empirical}.
\end{proof}

\subsubsection{Proof of \pref{lem:main-induction}}

Fix the $(x_{h-1}, a_{h-1})$ pair on which we call \stochdecoder.

For notational convenience we will denote $\cXL \coloneqq \cD$ and $\cXR \coloneqq \estmdpobsspace{h}$, as well as use $\optlatp = \optlatp(\cdot~|~\optdec(x_{h-1}), a_{h-1})$ to denote the ground truth latent transition function. Throughout the proof, we use $K>0$ to denote absolute constants whose values may change line-by-line. 

\paragraph{Part (1).} Since the input confidence set $\cP$ satisfies the third bullet, it suffices to show that that $\projm{\estmdpobsspace{h}}(\optlatp)$ satisfies both of the constraints in the confidence set construction of Eq.~\eqref{eq:confidence-set-construction-v2}.

For the first constraint, observe that by \pref{corr:estimating-projR},
\begin{align*}
    \sum_{\cc \in \crl{\cc_j}} \abs*{ \frac{\abs{\ccL}}{\abs{\cXL}} 
 - \projR(\samplelatp)(\ccR) } \le 2\eps.
\end{align*}
Therefore it suffices to show that 
\begin{align*}
    \sum_{\cc \in \crl{\cc_j}} \abs*{\projR(\optlatp)(\ccR) - \projR(\samplelatp)(\ccR) } \le \eps.
\end{align*}
We calculate that
\begin{align*}
    \hspace{2em}&\hspace{-2em} \sum_{\cc \in \crl{\cc_j}} \abs*{\projR(\optlatp)(\ccR) - \projR(\samplelatp)(\ccR)} \\
    &\le \sum_{\empobs \in \cXR}  \abs*{\projR(\optlatp)(\empobs) - \projR(\samplelatp)(\empobs)} \\
    &= \sum_{\empobs \in \cXR}  \abs*{\prn*{\optlatp(\optdec(\empobs)) - \samplelatp(\optdec(\empobs))} \cdot \frac{\ind{\optdec(\empobs) \in \epsPRS{}}}{n_{\optdec(\empobs)}[\cXR]}} \\
    &= \sum_{s \in \epsPRS{}} \sum_{\empobs \in \cXR}  \abs*{\prn*{\optlatp(s) - \samplelatp(s)} \cdot \frac{\ind{\optdec(\empobs) = s}}{n_{s}[\cXR]}} \\
    &= \sum_{s \in \epsPRS{}} \abs*{\optlatp(s) - \samplelatp(s) } \le \eps. &\text{(\pref{lem:sampling-transitions})} \numberthis \label{eq:bound-on-empirical-proj}
\end{align*}
Now we prove that $\projR(\optlatp)$ also satisfies the second constraint, i.e.,
\begin{align*}
    \sum_{\cc \in \crl{\cc_j}}  \frac{\abs{\ccL}}{\abs{\cXL}} \cdot \nrm*{\pi \push \unif(\ccL) - \pi \push \projR(\optlatp)(\cdot~|~\ccR) }_1 \le \eps.
\end{align*}

Observe that we can break up the bound as follows:
\begin{align*}
    \hspace{2em}&\hspace{-2em} \sum_{\cc \in \crl{\cc_j}}  \frac{\abs{\ccL}}{\abs{\cXL}} \cdot \nrm*{\pi \push \unif(\ccL) - \pi \push \projR(\optlatp)(\cdot~|~\ccR) }_1 \\
    &\le \underbrace{ \sum_{\cc \in \crl{\cc_j}}  \frac{\abs{\ccL}}{\abs{\cXL}} \cdot \nrm*{\pi \push \unif(\ccL) - \pi \push \projR(\samplelatp)(\cdot~|~\ccR) }_1 }_{\eqqcolon \mathtt{Term}_1}  \\
    &\hspace{5em} + \underbrace{\sum_{\cc \in \crl{\cc_j}}  \frac{\abs{\ccL}}{\abs{\cXL}} \cdot \nrm*{\pi \push \projR(\samplelatp)(\cdot~|~\ccR) - \pi \push \projR(\optlatp)(\cdot~|~\ccR) }_1 }_{\eqqcolon \mathtt{Term}_2}.
\end{align*}

To bound $\mathtt{Term}_1$, we compute:
\begin{align*}
    \hspace{2em}&\hspace{-2em} \sum_{\cc \in \crl{\cc_j}}  \frac{\abs{\ccL}}{\abs{\cXL}} \cdot \nrm*{\pi \push \unif(\ccL) - \pi \push \projR(\samplelatp)(\cdot~|~\ccR) }_1 \\
    &\le \sum_{\cc \in \crl{\cc_j}:  \frac{\abs{\ccL}}{\abs{\cXL}} \ge 4\eps}  \frac{\abs{\ccL}}{\abs{\cXL}} \cdot \nrm*{\pi \push \unif(\ccL) - \pi \push \projR(\samplelatp)(\cdot~|~\ccR) }_1 + \sum_{\cc \in \crl{\cc_j} :  \frac{\abs{\ccL}}{\abs{\cXL}} < 4\eps }  \frac{2\abs{\ccL}}{\abs{\cXL}} \\
    &\overset{(i)}{\le} \sum_{\cc \in \crl{\cc_j}:  \frac{\abs{\ccL}}{\abs{\cXL}} \ge 4\eps}  \frac{\abs{\ccL}}{\abs{\cXL}} \cdot \nrm*{\pi \push \unif(\ccL) - \pi \push \projR(\samplelatp)(\cdot~|~\ccR) }_1 + (8S+4)\eps \\
    &\le  \sum_{\cc \in \crl{\cc_j} :  \frac{\abs{\ccL}}{\abs{\cXL}} \ge 4\eps }  \frac{\abs{\ccL}}{\abs{\cXL}} \cdot \prn*{ K \cdot \sqrt{\frac{S A^2 \log \tfrac{SA \abs{\Pi}}{\delta}}{\nrch[\ccL]}} + A \cdot \frac{\nurch[\ccL]}{\nrch[\ccL]} } + (8S+5)\eps &\hspace{-10em}\text{(\pref{lem:relating-proj-to-empirical})}\\
    &=  \sum_{\cc \in \crl{\cc_j} :  \frac{\abs{\ccL}}{\abs{\cXL}} \ge 4\eps }  \frac{\nrch[\ccL] + \nurch[\ccL]}{\abs{\cXL}} \cdot \prn*{ K \cdot \sqrt{\frac{S A^2 \log \tfrac{SA \abs{\Pi}}{\delta}}{\nrch[\ccL]}}  + A \cdot \frac{\nurch[\ccL]}{\nrch[\ccL]} } + (8S+5)\eps. \numberthis\label{eq:term1-intermediate}
\end{align*}
The inequality $(i)$ follows by casework on $\cc \in \crl{\cc_j}$:
\begin{itemize}
    \item If $\epsPRS{} \cap \cS[\ccL] \ne \emptyset$ then by the biclique lemma (\pref{lem:biclique}) we have $\crl{x \in \cXL: \optdec(x) \in \epsPRS{} \cap \cS[\ccL]} \subseteq \ccL$. In other words, all of the observations from states in $\epsPRS{} \cap \cS[\ccL]$ are contained in $\ccL$. Therefore, there can be at most $S$ such components $\cc$, and their contribution to the sum is $8\eps \cdot S$.
    \item If $\epsPRS{} \cap \cS[\ccL] = \emptyset$, then $\ccL$ only contains observations from $(\epsPRS{})^c$, and therefore the total size of such $\ccL$ can be bounded by $2\eps$ using \pref{corr:sampling-transitions}. Their contribution to the sum is $4\eps$.
\end{itemize}
We now proceed to separately bound the terms in Eq.~\eqref{eq:term1-intermediate}. First, observe that
\begin{align*}
    K \sqrt{SA^2 \log \tfrac{SA \abs{\Pi}}{\delta}}\cdot \sum_{\cc \in \crl{\cc_j}: \frac{\abs{\ccL}}{\abs{\cXL}} \ge 4\eps}  \frac{\sqrt{\nrch[\ccL]} }{\abs{\cXL}}  &\le K \sqrt{\frac{S^2A^2 \log \tfrac{SA \abs{\Pi}}{\delta}}{\nrch[\cXL]}} \\
    &\le K \sqrt{\frac{S^2A^2 \log \tfrac{ SA \abs{\Pi}}{\delta}}{\ndec}} \\
    &\le \eps. \numberthis \label{eq:term1-intermediate2}
\end{align*}
The first inequality follows because by the biclique lemma (\pref{lem:biclique}) we know that the summation must have at most $S$ terms, since each of the $\cc$ contains some $s \in \epsPRS{}$, so we can apply Cauchy-Schwarz for $S$-dimensional vectors. The second inequality is a consequence of \pref{corr:sampling-transitions}, and the last inequality follows by our choice of $\ndec$.

In addition by \pref{corr:sampling-transitions},
\begin{align*}
    \sum_{\cc \in \crl{\cc_j}: \frac{\abs{\ccL}}{\abs{\cXL}} \ge 4\eps }  \frac{\nrch[\ccL] }{\abs{\cXL}} \frac{\nurch[\ccL]}{\nrch[\ccL]} \le 2\eps. \numberthis \label{eq:term1-intermediate3}
\end{align*}
For the other two terms, observe that when $ \frac{\abs{\ccL}}{\abs{\cXL}} \ge 4\eps$ we must have $\frac{\nurch[\ccL]}{\nrch[\ccL]} \le 1$ so therefore
\begin{align*}
    \hspace{2em}&\hspace{-2em} \sum_{\cc \in \crl{\cc_j} : \frac{\abs{\ccL}}{\abs{\cXL}} \ge 4\eps}  \frac{\nurch[\ccL]}{\abs{\cXL}} 
  \prn*{ K \cdot \sqrt{\frac{SA^2 \log \tfrac{SA \abs{\Pi}}{\delta}}{\nrch[\ccL]}}+ \frac{\nurch[\ccL]}{\nrch[\ccL]} } \\
  &\le \sum_{\cc \in \crl{\cc_j}: \frac{\abs{\ccL}}{\abs{\cXL}} \ge 4\eps} \frac{\nurch[\ccL]}{\abs{\cXL}} 
  \prn*{ K \cdot \sqrt{SA^2 \log \frac{ SA \abs{\Pi}}{\delta} } +1} \\
  &\le K \sqrt{SA^2 \log \frac{ SA \abs{\Pi}}{\delta} } \cdot \eps. \numberthis \label{eq:term1-intermediate4}
\end{align*}
Combining Eqns.~\eqref{eq:term1-intermediate}, \eqref{eq:term1-intermediate2}, \eqref{eq:term1-intermediate3}, and \eqref{eq:term1-intermediate4} we get that
\begin{align*}
    \sum_{\cc \in \crl{\cc_j}}  \frac{\abs{\ccL}}{\abs{\cXL}} \cdot \nrm*{\pi \push \unif(\ccL) - \pi \push \projR(\samplelatp)(\cdot~|~\ccR) }_1 \le K \prn*{  \sqrt{SA^2 \log \frac{ SA \abs{\Pi}}{ \delta} } + S}\eps. \numberthis \label{eq:term1-final}
\end{align*}
To bound $\mathtt{Term}_2$, fix any $\cc \in \crl{\cc_j}$. Note that
\begin{align*}
     \hspace{2em}&\hspace{-2em} \nrm*{\pi \push \projR(\optlatp)(\cdot~|~\ccR) - \pi\push \projR(\samplelatp)(\cdot~|~\ccR)}_1 \\
     &= \sum_{a \in \cA} \abs*{\sum_{\empobs \in \ccR} \prn*{ \frac{\projR(\samplelatp)(\empobs)}{\projR(\samplelatp)(\ccR)}  - \frac{\projR(\optlatp)(\empobs)}{\projR(\optlatp)(\ccR)} }\indd{\pi(\empobs) = a}}\\
     &\le \sum_{\empobs \in \ccR} \abs*{ \frac{\projR(\samplelatp)(\empobs)}{\projR(\samplelatp)(\ccR)}  - \frac{\projR(\optlatp)(\empobs)}{\projR(\optlatp)(\ccR)} } \\
     &=  \sum_{\empobs \in \ccR} \abs*{ \frac{ \samplelatp(\optdec(\empobs))}{\projR(\samplelatp)(\ccR)}  - \frac{\optlatp(\optdec(\empobs))}{\projR(\optlatp)(\ccR)} } \cdot \frac{\ind{\optdec(\empobs) \in \epsPRS{}}}{n_{\optdec(\empobs)}[\cXR]} \\
     &= \sum_{s \in \epsPRS{} \cap \cS[\ccL] \cap \cS[\ccR]} \abs*{ \frac{ \samplelatp(s)}{\projR(\samplelatp)(\ccR)}  - \frac{ \optlatp(s)}{\projR(\optlatp)(\ccR)} } \\
     &=  \frac{ 1 }{\projR(\samplelatp)(\ccR)}\sum_{s \in \epsPRS{} \cap \cS[\ccL] \cap \cS[\ccR]} \abs*{ \samplelatp(s) - \optlatp(s) \cdot \frac{ \projR(\samplelatp)(\ccR)}{\projR(\optlatp)(\ccR)} } \\
     &\le \frac{ \eps }{\projR(\samplelatp)(\ccR)} + \frac{ 1 }{\projR(\samplelatp)(\ccR)}\sum_{s \in \epsPRS{} \cap \cS[\ccL] \cap \cS[\ccR]}\optlatp(s) \abs*{ 1 - \frac{\projR(\samplelatp)(\ccR)}{\projR(\optlatp)(\ccR)} } &\text{(\pref{lem:sampling-transitions})}\\
     &= \frac{ \eps }{\projR(\samplelatp)(\ccR)} +  \frac{ 1 }{\projR(\samplelatp)(\ccR)} \abs*{\projR(\optlatp)(\ccR)  -  \projR(\samplelatp)(\ccR) } \\
     &\le \frac{ 2\eps }{\projR(\samplelatp)(\ccR)} =  2\eps \frac{\abs{\cXL} }{\nrch[\ccL]}. &\text{(using Eq.~\pref{eq:bound-on-empirical-proj})} \numberthis\label{eq:term2}
\end{align*}
Using Eq.~\pref{eq:term2} and \pref{corr:sampling-transitions} we get that
\begin{align*}
    \sum_{\cc \in \crl{\cc_j}}  \frac{\abs{\ccL}}{\abs{\cXL}} \cdot \nrm*{\pi \push \projR(\samplelatp)(\cdot~|~\ccR) - \pi \push \projR(\optlatp)(\cdot~|~\ccR) }_1 \le \sum_{\cc \in \crl{\cc_j}}  \frac{\abs{\ccL}}{\abs{\cXL}} \cdot 2\eps \frac{\abs{\cXL} }{\nrch[\ccL]} \le 4\eps. \numberthis \label{eq:final-bound-term2}
\end{align*}

Putting together Eqns.~\eqref{eq:term1-final} and \eqref{eq:final-bound-term2}:
\begin{align*}
    \sum_{\cc \in \crl{\cc_j}}  \frac{\abs{\ccL}}{\abs{\cXL}} \cdot \nrm*{\pi \push \unif(\ccL) - \pi \push \projR(\optlatp)(\cdot~|~\ccR) }_1 &\le K \prn*{  \sqrt{SA^2 \log \frac{SA  \abs{\Pi}}{\delta} }+ S}\eps \eqqcolon \beta.
\end{align*}
Thus, we can conclude that $\projR(\optlatp) \in \cP$, thus concluding the proof of Part (1).

\paragraph{Part (2).} Observe that in light of Part (1), the set $\cP$ is nonempty so therefore the maximum is well defined.

We want to show a bound on
\begin{align*}
    \max_{\bar{p} \in \cP} \max_{\pi \in \Pi_{h:H}}~\abs*{Q^\pi(x_{h-1},a_{h-1}) - \wh{R}(x_{h-1},a_{h-1}) - \En_{\empobs_{h} \sim \bar{p}} \wh{V}^\pi(\empobs_{h})}.
\end{align*}

Fix any $\bar{p} \in \cP$ and $\pi \in \Pi_{h:H}$. We compute
\begin{align*}
    \hspace{2em}&\hspace{-2em} \abs*{Q^\pi(x_{h-1},a_{h-1}) - \wh{R}(x_{h-1},a_{h-1}) - \En_{\empobs_{h} \sim \bar{p}} \wh{V}^\pi(\empobs_{h})} \\
    &\le \frac{\eps}{H} + \abs*{ \En_{s_h \sim \optlatp} V^\pi(s_h) - \En_{s_{h} \sim \samplelatp} V^\pi(s_{h}) } + \abs*{ \En_{s_{h} \sim \samplelatp} V^\pi(s_{h}) - \En_{\empobs_{h} \sim \bar{p}} \wh{V}^\pi(\empobs_{h}) } &\hspace{-10em}\text{(\pref{lem:sampling-rewards})}\\
    &\le 2\eps + \abs*{ \En_{s_{h} \sim \samplelatp} V^\pi(s_{h}) - \En_{\empobs_{h} \sim \bar{p}} \wh{V}^\pi(\empobs_{h}) } &\hspace{-10em}\text{(\pref{lem:sampling-transitions})} \\
    &\le 2\eps + \underbrace{ \abs*{ \En_{s_{h} \sim \samplelatp} V^\pi(s_{h}) - \En_{\empobs_{h} \sim \projR(\samplelatp)} V^\pi(\empobs_{h}) } }_{ \eqqcolon \mathtt{Term}_1} + \underbrace{ \abs*{ \En_{\empobs_{h} \sim \projR(\samplelatp)} V^\pi(\empobs_{h}) - \En_{\empobs_{h} \sim \projR(\samplelatp)} \wh{V}^\pi(\empobs_{h})} }_{\eqqcolon \mathtt{Term}_2} \\
    &\quad\quad + \underbrace{ \abs*{\En_{\empobs_{h} \sim \projR(\samplelatp)} \wh{V}^\pi(\empobs_{h}) - \En_{\empobs_{h} \sim \bar{p}} \wh{V}^\pi(\empobs_{h}) } }_{\eqqcolon \mathtt{Term}_3}
\end{align*}
For the first term, we can calculate that
\begin{align*}
    \mathtt{Term}_1 &= \abs*{ \En_{s_{h} \sim \samplelatp} V^\pi(s_{h}) - \En_{\empobs_{h} \sim \projR(\samplelatp)} V^\pi(\empobs_{h}) } \\
    &= \abs*{ \En_{s_{h} \sim \samplelatp} \En_{x_{h} \sim \emission(s_{h}) } V^\pi(x_{h}) - \En_{\empobs_{h} \sim \projR(\samplelatp)} V^\pi(\empobs_{h}) } \\
    &= \abs*{ \En_{s_{h} \sim \samplelatp} \brk*{ \En_{x_{h} \sim \emission(s_{h}) } V^\pi(x_{h}) - \En_{\empobs_{h} \sim \mathrm{Unif}(\crl{\empobs_{h} \in \cXR: \optdec(\empobs_{h}) = s_{h}})} V^\pi(\empobs_{h}) } } \\
    &\le 2\eps + \abs*{ \En_{s_{h} \sim \samplelatp} \brk*{ \ind{s_{h} \in \epsPRS{h}} \prn*{ \En_{x_{h} \sim \emission(s_{h}) } V^\pi(x_{h}) - \En_{\empobs_{h} \sim \mathrm{Unif}(\crl{\empobs_{h}\in \cXR: \optdec(\empobs_{h}) = s_{h}})} V^\pi(\empobs_{h}) } } } \\
    &\le 3\eps. \numberthis\label{eq:t1}
\end{align*}
The first inequality follows by \pref{corr:sampling-transitions}, and the second inequality follows by \pref{lem:pushforward-concentration}.

\glcomment{this needs to be modified for the concentrability setting.} For the second term, we have by assumption that:
\begin{align*}
    \mathtt{Term}_2 = \abs*{ \En_{\empobs_{h} \sim \projR(\samplelatp)} \brk*{V^\pi(\empobs_{h}) - \wh{V}^\pi(\empobs_{h})}  } \le \Gamma_{h}. \numberthis\label{eq:t2}
\end{align*}

Now we calculate a bound on $\mathtt{Term}_3$. In what follows for any connected component $\cc$ we let $\empobs_\cc$ denote an arbitrary fixed observation from $\ccR$ (for example, the lowest indexed one). Observe that for any $p \in \Delta(\cXR)$ we have
\begin{align*}
    \En_{\empobs \sim p} \wh{V}^\pi(\empobs) 
    &= \sum_{\cc\in \crl{\cc_j}} \sum_{\empobs \in \ccR} p(\empobs) \cdot \wh{Q}^\pi(\empobs, \pi(\empobs)) &\text{($\crl{\cc_j}$ form a partition of $\cXR$)}\\
    &\le 4S\taudec + 8S\eps +  \sum_{\cc \in \crl{\cc_j}} \sum_{\empobs \in \ccR} p(\empobs) \cdot \wh{Q}^\pi(\empobs_\cc, \pi(\empobs_\cc)) &\text{(\pref{lem:width-of-cc})}\\
    &= 4S\taudec + 8S\eps +  \sum_{\cc \in \crl{\cc_j}} p(\ccR) \sum_{\empobs \in \ccR} \frac{p(\empobs)}{p(\ccR)} \wh{Q}^\pi(\empobs_\cc, \pi(\empobs_\cc)).
\end{align*}
Similarly, one can show the lower bound on $\En_{\empobs \sim p} \wh{V}^\pi(\empobs)$. Therefore we apply the bound to get:
\begin{align*}
    \hspace{2em}&\hspace{-2em} \abs*{\En_{\empobs \sim \projR(\samplelatp)} \wh{V}^\pi(\empobs) - \En_{\empobs \sim \bar{p}} \wh{V}^\pi(\empobs) } \\
    &\le 8S\taudec + 16S\eps + \sum_{\cc \in \crl{\cc_j}} \abs*{\projR(\samplelatp)(\ccR) \sum_{\empobs \in \ccR} \frac{\projR(\samplelatp)(\empobs)}{\projR(\samplelatp)(\ccR) } \wh{Q}^\pi(\empobs_\cc, \pi(\empobs)) - \bar{p}(\cc) \sum_{\empobs \in \ccR} \frac{\bar{p}(\empobs)}{\bar{p}(\cc)} \wh{Q}^\pi(\empobs_\cc, \pi(\empobs)) } \\
    &\overset{(i)}{\le} 8S\taudec + 16S\eps + 2\eps + \sum_{\cc \in \crl{\cc_j}} \abs*{\frac{\abs{\ccL}}{\abs{\cXL}} \sum_{\empobs \in \cc} \frac{\projR(\samplelatp)(\empobs)}{\projR(\samplelatp)(\ccR) } \wh{Q}^\pi(\empobs_\cc, \pi(\empobs)) - \bar{p}(\cc) \sum_{\empobs \in \cc} \frac{\bar{p}(\empobs)}{\bar{p}(\cc)} \wh{Q}^\pi(\empobs_\cc, \pi(\empobs)) } \\
    &\overset{(ii)}{\le}  8S\taudec + 16S\eps + 5\eps + \sum_{\cc \in \crl{\cc_j}}  \frac{\abs{\ccL}}{\abs{\cXL}} \cdot \abs*{\sum_{\empobs \in \cc} \frac{\projR(\samplelatp)(\empobs)}{\projR(\samplelatp)(\ccR) } \wh{Q}^\pi(\empobs_\cc, \pi(\empobs)) - \frac{\bar{p}(\empobs)}{\bar{p}(\cc)} \wh{Q}^\pi(\empobs_\cc, \pi(\empobs)) },\\
    &\le 8S\taudec + 16S\eps + 5\eps + \sum_{\cc \in \crl{\cc_j}}  \frac{\abs{\ccL}}{\abs{\cXL}} \cdot \nrm*{\pi\push \projR(\samplelatp)(\cdot~|~\ccR) - \pi \push \bar{p}(\cdot~|~\cc) }_1 ,
\end{align*}
where $(i)$ follows by \pref{corr:estimating-projR} and the bound $\frac{\projR(\samplelatp)(\empobs)}{\projR(\samplelatp)(\ccR) } \wh{Q}^\pi(\empobs_\cc, \pi(\empobs)) \in [0,1]$, and $(ii)$ follows by the first constraint on $\bar{p} \in \cP$ and the bound $\frac{p(\empobs)}{p(\cc)} \wh{Q}^\pi(\empobs_\cc, \pi(\empobs)) \in [0,1]$. 

From here, we will use the second constraint on $\bar{p} \in \cP$:
\begin{align*}
    \hspace{2em}&\hspace{-2em}  \abs*{\En_{\empobs \sim \projR(\samplelatp)} \wh{V}^\pi(\empobs) - \En_{\empobs \sim \bar{p}} \wh{V}^\pi(\empobs) } \\
    &\le  8S\taudec + 16S\eps + 5\eps + \sum_{\cc \in \crl{\cc_j}}  \frac{\abs{\ccL}}{\abs{\cXL}} \cdot \nrm*{\pi\push \projR(\samplelatp)(\cdot~|~\ccR) - \pi \push \bar{p}(\cdot~|~\cc) }_1 \\
    &\le  8S\taudec + 16S\eps + 5\eps + \beta + \sum_{\cc \in \crl{\cc_j}}  \frac{\abs{\ccL}}{\abs{\cXL}} \cdot \nrm*{\pi\push \projR(\samplelatp)(\cdot~|~\ccR) -\pi \push \unif(\ccL) }_1 \\
    &\le  8S\taudec + 16S\eps + 5\eps + 2\beta. \numberthis\label{eq:t3}
\end{align*}
The last inequality follows because our proof for Part (1) of the lemma actually showed that $\projR(\samplelatp) \in \cP$. Combining Eqns.~\eqref{eq:t1}, \eqref{eq:t2}, and \eqref{eq:t3} we get the final bound
\begin{align*}
    \abs*{Q^\pi(x_{h-1},a_{h-1}) - \wh{R}(x_{h-1},a_{h-1}) - \En_{\empobs_{h} \sim \bar{p}} \wh{V}^\pi(\empobs_{h})} \le \Gamma_h + K \cdot \prn*{\beta + S \taudec}.
\end{align*}
This completes the proof of \pref{lem:main-induction}.

\subsection{Analysis of \stochrefit}
\glcomment{for refitting, we need to delete states which have been updated too many times. show that these states must not be eps-reachable.}
\begin{lemma}[Certificate Implies Transition Inaccuracy]\label{lem:certificate-obs}
Assume that $\eventemulator$ hold. Let $\wh{M}$ be a policy emulator, and let $\tau > 2\eps$ be a parameter. Suppose there exists a certificate $(\empobs, \pi) \in \cX[\wh{M}] \times (\cA \circ \Pi)$ such that
\begin{align*}
    \abs*{\wh{V}^{\pi}(\empobs) - V^{\pi}(\empobs)} \ge \tau.
\end{align*}
Then there exists some tuple $(\bar{\empobs}, \bar{a}) \in \estmdpobsspace{} \times \actionsp$ such that
\begin{align*}
    \abs*{\En_{\empobs' \sim \wh{P}(\cdot~|~ \bar{\empobs}, \bar{a})} V^{\pi}(\empobs') - \En_{\empobs' \sim P(\cdot~|~ \bar{\empobs}, \bar{a})} V^{\pi}(\empobs')} \ge \frac{\tau}{2H}. \numberthis\label{eq:bad-state}
\end{align*}
\end{lemma}

\begin{proof}Let $h = h(\empobs)$ be the layer that $\empobs$ is found in. Suppose that Eq.~\eqref{eq:bad-state} did not hold for any $(\bar{\empobs}, \bar{a})$. Then by the Performance Difference Lemma we have
\begin{align*}
    \hspace{2em}&\hspace{-2em} \abs*{ V^{\pi}(\empobs) - \wh{V}^{\pi}(\empobs) } \\
    &\le \abs*{\wh{R}(x, \pi) - R(x,\pi)} + \abs*{ \En_{s' \sim P(\cdot~|~\empobs, \pi)} V^{\pi}(s') - \En_{\empobs' \sim \wh{P}(\cdot~|~\empobs, \pi)}V^{\pi}(\empobs') } \\
    &\hspace{5em} + \abs*{\En_{\empobs' \sim \wh{P}(\cdot~|~\empobs, \pi)}V^{\pi}(\empobs') - \En_{\empobs' \sim \wh{P}(\cdot~|~\empobs, \pi)} \wh{V}^{\pi}(\empobs') }\\
    &\le \frac{\tauref}{2H} + \frac{\eps}{H} + \abs*{\En_{\empobs' \sim \wh{P}(\cdot~|~\empobs, \pi)}V^{\pi}(\empobs') - \En_{\empobs' \sim \wh{P}(\cdot~|~\empobs, \pi)} \wh{V}^{\pi}(\empobs') } &\text{(\pref{lem:sampling-rewards} and neg.~of Eq.~\eqref{eq:bad-state})}\\
    &\le \frac{\tauref}{2H} + \frac{\eps}{H} + \max_{\empobs' \in \estmdpobsspace{h+1}}\abs*{  V^{\pi}(\empobs') - \wh{V}^{\pi}(\empobs') } \\
    &\le \cdots \\
    &\le \frac{\tauref}{2} + \eps. &\text{(Recursion)}
\end{align*}
Thus, we have reached a contradiction. This proves \pref{lem:certificate-obs}.
\end{proof}

\begin{lemma}[Refitting Correctness]\label{lem:refitting-correctness} Assume that $\eventemulator, \eventref$ hold. The following are true about \pref{alg:stochastic-refit-v2} in the search for incorrect transitions (\pref{line:else-triggered}-\ref{line:loss-vector-obs} are executed):
\begin{enumerate}
    \item[(1)] For every $(\empobs, \pi)$ from in \pref{line:for-every}, at least one such $(\bar{\empobs}, \bar{a})$ pair is identified by \pref{line:bad-obs-stochastic}.
    \item[(2)] Every $(\bar{\empobs}, \bar{a})$ pair identified by \pref{line:bad-obs-stochastic} satisfies
    \begin{align*}
    \abs*{\En_{\empobs' \sim \wh{P}(\cdot~|~\bar{\empobs}, \bar{a})} V^{\pi}(\empobs') - \En_{\empobs' \sim \projm{\estmdpobsspace{h(\bar{\empobs})+1}}(\optlatp) } V^\pi(\empobs') } \ge \frac{\tauref}{16H}.
    \end{align*}
    \item[(3)] For every $(\bar{\empobs}, \bar{a})$ identified by \pref{line:bad-obs-stochastic}, the corresponding loss vector $\ell_\mathrm{loss}$ from \pref{line:loss-vector-obs} satisfies
    \begin{align*}
        \tri*{\wh{P}(\cdot~|~\bar{\empobs}, \bar{a}) - \projm{\estmdpobsspace{h(\bar{\empobs})+1}}(\optlatp(\cdot~|~\bar{\empobs}, \bar{a})), \ell_\mathrm{loss} } \ge \frac{\tauref}{16H}.
    \end{align*}
\end{enumerate}
\end{lemma}

\begin{proof}
To prove Part (1) we use \pref{lem:certificate-obs}, which shows that there exists at least one such $(\bar{\empobs}, \bar{a})$ such that
\begin{align*}
    \abs*{\En_{\empobs' \sim \wh{P}(\cdot~|~ \bar{\empobs}, \bar{a})} V^{\pi}(\empobs') - \En_{\empobs' \sim P(\cdot~|~ \bar{\empobs}, \bar{a})} V^{\pi}(\empobs')} \ge \frac{\tauref}{2H}. \numberthis\label{eq:lower-bound}
\end{align*}
Therefore we know that for such $(\bar{\empobs}, \bar{a})$:
\begin{align*}
    &\abs*{\En_{\empobs' \sim \wh{P}(\cdot~|~ \bar{\empobs}, \bar{a})} V^{\pi}(\empobs') - \En_{\empobs' \sim P(\cdot~|~ \bar{\empobs}, \bar{a})} V^{\pi}(\empobs')} \\
    &\le \abs*{\En_{\empobs' \sim \wh{P}(\cdot~|~ \bar{\empobs}, \bar{a})} \vest(\pi;\empobs') + \wh{R}(\bar{\empobs}, \bar{a}) - \qest(\pi; \bar{\empobs}, \bar{a})} + 3\eps &\text{(\pref{lem:refit-monte-carlo-accuracy} and \pref{lem:sampling-rewards})}\\
    &= \abs*{ \Delta(\bar{\empobs}, \bar{a}) } + 3\eps \\
    &\Longrightarrow  \quad \abs*{ \Delta(\bar{\empobs}, \bar{a}) } \ge \frac{\tauref}{2H} - 3\eps \ge \frac{\tauref}{8H}. &\text{(Using Eq.~\eqref{eq:lower-bound})}
\end{align*}
so therefore this $(\bar{\empobs}, \bar{a})$ is identified by \pref{line:bad-obs-stochastic} of \stochrefit{}.

Now we prove Part (2). Fix any $(\bar{\empobs}, \bar{a})$ pair identified by \pref{line:bad-obs-stochastic} of \stochrefit{}. Let $h=h(\bar{\empobs})$ denote the layer that a given $\bar{\empobs}$ is found. First we observe that
\begin{align*}
    \hspace{2em}&\hspace{-2em} \En_{\empobs' \sim P(\cdot~|~ \bar{\empobs}, \bar{a})} V^{\pi}(\empobs') - \En_{\empobs' \sim \projm{\estmdpobsspace{h+1}}(\optlatp) } V^\pi(\empobs') \\
    &= \En_{\empobs' \sim \emission \circ \optlatp } V^\pi(\empobs') - \En_{\empobs' \sim \projm{\estmdpobsspace{h+1}}(\optlatp) } V^\pi(\empobs') \\
    &= \En_{s \sim \optlatp} \brk*{\En_{\empobs' \sim \emission(s) } \brk*{ V^\pi(\empobs') } - \ind{s \in \epsPRS{}} \En_{\empobs' \sim \mathrm{Unif}(\crl{\empobs \in \estmdpobsspace{h+1}: \optdec(\empobs) = s})} \brk*{V^\pi(\empobs')} }\\
    &\le \eps + \En_{s \sim \optlatp} \brk*{\ind{s \in \epsPRS{}} \prn*{ \En_{\empobs' \sim \emission(s) } \brk*{ V^\pi(\empobs') } -  \En_{\empobs' \sim \mathrm{Unif}(\crl{\empobs\in \estmdpobsspace{h+1}: \optdec(\empobs) = s})} \brk*{V^\pi(\empobs')} } } \\
    &\le 2\eps,
\end{align*}
where the last inequality uses \pref{lem:pushforward-concentration}. The other side of the inequality can be similarly shown, so
\begin{align*}
    \abs*{ \En_{\empobs' \sim P(\cdot~|~ \bar{\empobs}, \bar{a})} V^{\pi}(\empobs') - \En_{\empobs' \sim \projm{\estmdpobsspace{h+1}}(\optlatp) } V^\pi(\empobs') }
    \le 2\eps. \numberthis \label{eq:relating-q-to-proj}
\end{align*}
We can compute that
\begin{align*}
    \frac{\tauref}{8H} &\le \abs{ \Delta(\bar{\empobs}, \bar{a}) } \\
    &=  \abs*{\En_{\empobs' \sim \wh{P}(\cdot~|~ \bar{\empobs}, \bar{a})} \vest(\pi;\empobs') + \wh{R}(\bar{\empobs}, \bar{a}) - \qest(\pi; \bar{\empobs}, \bar{a})} \\
    &\le \abs*{\En_{\empobs' \sim \wh{P}(\cdot ~|~ \bar{\empobs},\bar{a})} V^\pi(\empobs') + \wh{R}(\bar{\empobs}, \bar{a}) - Q^\pi(\bar{\empobs}, \bar{a})} + 2\eps &\text{(\pref{lem:refit-monte-carlo-accuracy})} \\
    &\le \abs*{\En_{\empobs' \sim \wh{P}(\cdot ~|~ \bar{\empobs},\bar{a})} V^\pi(\empobs') - \En_{\empobs' \sim P(\cdot~|~ \bar{\empobs}, \bar{a})} V^{\pi}(\empobs') } + 3\eps &\text{(\pref{lem:sampling-rewards})} \\
    &\le \abs*{ \En_{\empobs' \sim \wh{P}(\cdot ~|~ \bar{\empobs},\bar{a})} V^\pi(\empobs') -\En_{\empobs' \sim \projm{\estmdpobsspace{h+1}}(\optlatp) } V^\pi(\empobs') } + 5\eps. &\text{(Eq.~\eqref{eq:relating-q-to-proj})}
\end{align*}
Rearranging we see that
\begin{align*}
    \abs*{ \En_{\empobs' \sim \wh{P}(\cdot ~|~ \bar{\empobs},\bar{a})} V^\pi(\empobs') -\En_{\empobs' \sim \projm{\estmdpobsspace{h+1}}(\optlatp) } V^\pi(\empobs') } \ge \frac{\tauref}{8H} - 5\eps \ge \frac{\tauref}{16H},
\end{align*}
and this proves Part (2).

For Part (3), suppose that $\Delta(\bar{\empobs}, \bar{a}) \ge \tauref/8H$ (the case where $\Delta(\bar{\empobs}, \bar{a}) \le -\tauref/8H$ can be tackled similarly). Then we have $\ell_\mathrm{loss} \coloneqq \vest(\pi; \cdot) \in [0,1]^{\estmdpobsspace{h+1}}$. We can compute that
\begin{align*}
\frac{\tauref}{8H} &\le \En_{\empobs' \sim \wh{P}(\cdot~|~ \bar{\empobs}, \bar{a})} \vest(\pi;\empobs') + \wh{R}(\bar{\empobs}, \bar{a}) - \qest(\pi; \bar{\empobs}, \bar{a}) \\
&= \tri*{ \wh{P}(\cdot ~|~ \bar{\empobs},\bar{a}), \ell_\mathrm{loss}} + \wh{R}(\bar{\empobs}, \bar{a}) - \qest(\pi; \bar{\empobs}, \bar{a})  \\
&\le \eps + \tri*{ \wh{P}(\cdot ~|~ \bar{\empobs},\bar{a}), \ell_\mathrm{loss}} + \wh{R}(\bar{\empobs}, \bar{a}) - Q^\pi(\bar{\empobs}, \bar{a}) &\text{(\pref{lem:refit-monte-carlo-accuracy})}\\
&\le 4\eps + \tri*{ \wh{P}(\cdot ~|~ \bar{\empobs},\bar{a}), \ell_\mathrm{loss}} - \En_{\empobs' \sim \projm{\estmdpobsspace{h+1}}(\optlatp) } V^\pi(\empobs') &\text{(\pref{lem:sampling-rewards} and Eq.~\eqref{eq:relating-q-to-proj})}\\
&\le 5\eps + \tri*{ \wh{P}(\cdot ~|~ \bar{\empobs},\bar{a}) -  \projm{\estmdpobsspace{h+1}}(\optlatp(\cdot ~|~ \bar{\empobs},\bar{a})), \ell_\mathrm{loss}} &\text{(\pref{lem:refit-monte-carlo-accuracy})}
\end{align*}
Rearranging we get $ \tri*{ \wh{P}(\cdot ~|~ \bar{\empobs},\bar{a}) -  \projm{\estmdpobsspace{h+1}}(\optlatp(\cdot ~|~ \bar{\empobs},\bar{a})), \ell_\mathrm{loss}}  \ge \tauref/(16H)$, thus proving part (3).
\end{proof}

\begin{lemma}[Bound on Number of Refits]\label{lem:bound-on-number-refits}
Assume that $\eventemulator, \eventref$ hold, and that every time \pref{alg:stochastic-refit-v2} is called, the confidence sets $\cP$ satisfy 
\begin{align*}
    \forall~(x,a) \in \estmdpobsspace{}\times \cA: \quad \projm{\estmdpobsspace{h(x)}}(\optlatp(\cdot ~|~ x, a)) \in \cP(x, a).
\end{align*}
Then across all calls to \pref{alg:stochastic-refit-v2}, \pref{line:loss-vector-obs} is executed at most $(\nreset AH/ \eps^2) \cdot \log \nreset$ times.
\end{lemma}  
    
\begin{proof}
Fix $h \in [H]$ and a pair $(\empobs, a) \in \estmdpobsspace{h} \times \cA$. Suppose we execute \pref{line:loss-vector-obs} for $T_\mathrm{refit}$ times on $(\empobs, a)$. Denote the sequence of transition estimates as $\crl{\wh{P}^{(t)}(\cdot~|~x, a)}_{t \in [T_\mathrm{refit}]}$ and the sequence of loss vectors as $\crl{\ell_\mathrm{loss}^{(t)}}_{t \in [T_\mathrm{refit}]}$.
    
    By Part (3) of \pref{lem:refitting-correctness}, for all times $t \in [T_\mathrm{refit}]$,
    \begin{align*}
        \tri*{\wh{P}^{(t)}(\cdot~|~ x, a) - \projm{\estmdpobsspace{h+1}}(\optlatp(\cdot~|~x,a)), \ell_\mathrm{loss}^{(t)} } \ge \frac{\tauref}{16H}. \numberthis \label{eq:refit-lb-obs}
    \end{align*}
    On the other hand, we have a bound on the total regret of online gradient descent:
    \begin{align*}
        \sum_{t=1}^{T_\mathrm{refit}} \tri*{\wh{P}^{(t)}(\cdot~|~x,a) - \projm{\estmdpobsspace{h+1}}(\optlatp(\cdot~|~x,a)), \ell_\mathrm{loss}^{(t)} } \le 2\sqrt{\log \abs{\estmdpobsspace{h+1}} \cdot T_\mathrm{refit}}.\numberthis \label{eq:refit-ub-obs}
    \end{align*}
    Therefore, combining Eqs.~\eqref{eq:refit-lb-obs} and \eqref{eq:refit-ub-obs} we have the bound
    \begin{align*}
        T_\mathrm{refit} \le 2^{10} \cdot \frac{ H^2 \log \abs{\estmdpobsspace{h+1}}}{\tauref^2} \le \frac{\log \nreset}{\eps^2}.
    \end{align*}
    Using the fact that there are $\nreset AH$ such $(\empobs, a)$ pairs proves the result.
\end{proof}

\subsection{Proof of \pref{thm:pushforward-bmdp-result}}

In the proof, we will assume that $\eventemulator$ holds, that $\eventdec_t$ holds for all times $t \in [T_\mathsf{D}]$, that $\eventref_t$ holds for all times $t \in [T_\mathsf{R}]$. By union bound, this holds with probability at least $1-(3 T_\mathsf{D} + T_\mathsf{R} + 1) \delta$. 

We will show that under the choice of parameters $\nreset$, $\ndec$, and $\nmc$ in the algorithm pseudocode, \stochalg{} returns a $\wt{O}(SAH^2 \eps)$-optimal policy, and that $T_\mathsf{D}, T_\mathsf{R} \le \poly(\cpush, S,A, H, \eps^{-1}, \log \abs{\Pi}, \log \delta^{-1})$. Therefore, rescaling $\eps$ and $\delta$ will imply the final result.

\paragraph{Proof by Induction.} Take $\Gamma_h \coloneqq K (H-h+1) \prn{\beta +SH}\eps$ for some suitably large constant $K > 0$. Furthermore set $\taudec = 81 H \eps$. We will show that the following properties holds at every layer $h \in [H]$:
\begin{enumerate}
    \item [(1)] \textit{Transition set includes ground truth:} $\forall~ (x,a) \in \estmdpobsspace{h} \times \cA$, $\projm{\estmdpobsspace{h}}(\optlatp(\cdot ~|~ x,a)) \in \cP(x,a)$.
    \item [(2)] \textit{Accurate value estimates:} $\forall~ (x,a) \in \estmdpobsspace{h} \times \cA, \pi \in \Pi_{h+1:H}$, $\abs{Q^\pi(x,a) - \wh{Q}^\pi(x,a)} \le \Gamma_h$.
    \item [(3)] \textit{Valid test policies:} $\Pitest_h$ are $\taudec$-valid for $\estmdp$ at layer $h$.
\end{enumerate}

To analyze \stochalg{} we will show that at the end of every while loop, these properties always hold for all layers $h > \ell_\mathsf{next}$.

\underline{Base Case.} For the first loop with $\ell = H$, property (1) holds because there are no transitions to be constructed at layer $H$. By \pref{lem:sampling-rewards}, property (2) holds after the initialization of the policy emulator in \pref{line:init-end}. Furthermore, in the first call to \stochrefit{}, the computed test policies are open loop, so again using \pref{lem:sampling-rewards}, we see that \pref{line:great-success-stochastic} is triggered. Therefore, properties (2) and (3) hold at the end of the while loop. The current layer index is set to $\ell \gets H-1$.

\underline{Inductive Step.} Suppose the current layer index is $\ell$, and that properties (1)--(3) hold for all $h > \ell$. By \pref{lem:main-induction}, for every $(x_\ell, a_\ell)$ that we call \stochdecoder{} on the updated confidence sets $\cP$ returned by  satisfy property (1), and the choice $\wh{P} \in \cP$ satisfies property (2). Now we do casework on the outcome of \stochrefit{} called at layer $\ell$.

\begin{itemize}
    \item \textbf{Case 1: Return in \pref{line:great-success-stochastic}.}  By construction, property (3) is satisfied for layer $\ell$. In this case, since \stochrefit{} made no updates to $\estlatentmdp$ or $\cP$, properties (1) and (2) continue to hold at layer $\ell$ onwards.
    \item \textbf{Case 2: Return in \pref{line:great-success-stochastic-else}.} Property (1) holds because \stochrefit{} does not modify $\cP$. Let $\ell_\mathsf{next}$ denote the layer at which we jump to. \stochrefit{} made no updates to $\estlatentmdp$ at layers $\ell_\mathsf{next} + 1$ onwards, and therefore the previously computed test policies $\Pitest_{\ell_\mathsf{next}+1:H}$ must still be valid, so therefore properties (2) and (3) continue to hold at layer $\ell_\mathsf{next}$ onwards.
\end{itemize}

Continuing the induction, once $\ell \gets 0$ is reached in \stochalg{}, the policy emulator $\estmdp$ satisfies the bound
\begin{align*}
    \max_{\pi \in \Pi}~\abs*{V^\pi(s_1) - \En_{x_1 \sim \unif(\estmdpobsspace{1}) }\brk{\wh{V}^\pi(x_1)}} \le \Gamma_1 \le \wt{O}(SAH^2 \eps).\numberthis\label{eq:final-bound}
\end{align*}

\paragraph{Bounding the Number of Calls to \stochdecoder{} and \stochrefit{}.} By \pref{lem:bound-on-number-refits}, the total number of executions of \pref{line:loss-vector-obs} in \pref{alg:stochastic-refit-v2} is at most $\nreset AH \eps^{-2} \log \nreset$. In the worst case, every revisit to an already computed layer (i.e., jumping back to $\ell_\mathsf{next} \ge \ell$) requires us to restart \stochdecoder{} at layer $H$ and therefore decode at most $\nreset AH$ additional times, so therefore
\begin{align*}
    T_\mathsf{D} \le \frac{\nreset^2 A^2H^2}{\eps^2} \log \nreset.
\end{align*}
Similarly, every revisit in the worst case requires $H$ additional calls to \stochrefit{} so therefore
\begin{align*}
    T_\mathsf{R} \le \frac{\nreset A H^2}{\eps^2} \log \nreset.
\end{align*}
As claimed, both $T_\mathsf{D}$ and $T_\mathsf{R}$ are $\poly(\cpush, S,A, H, \eps^{-1}, \log \abs{\Pi}, \log \delta^{-1})$.

\paragraph{Final Sample Complexity Bound.} Now we compute the total number of samples.
\begin{itemize}
    \item \pref{alg:stochastic-bmdp-solver-v2} uses $\nreset \cdot AH$ samples to $\mu_h$ to form the state space of the policy emulator, and for each state-action pair we sample $\wt{O}(H^2\eps^{-2})$ times to estimate the reward.
    \item \pref{alg:stochastic-decoder-v2} is called $T_\mathsf{D} \le \wt{O}(\nreset^2 A^2 H^2 \eps^{-2})$  times, and each time we use $\ndec \cdot \nreset^2 \nmc$ rollouts.
    \item \pref{alg:stochastic-refit-v2} is called $T_\mathsf{R} \le \wt{O}(\nreset A H^2 \eps^{-2})$ times, and each time we use $2\nreset^2 \nmc$ to evaluate the test policies. Furthermore, by \pref{lem:bound-on-number-refits}, \pref{line:mc2} is triggered at most $\wt{O}(\nreset A H \eps^{-2})$ times, with every time requiring an additional $\nmc \cdot \nreset AH$ rollouts.
\end{itemize}

Therefore in total we use
\begin{align*}
     \hspace{2em}&\hspace{-2em} \nreset \frac{AH^3}{\eps^2} + \nreset^4 \ndec \nmc \frac{A^2H^2}{\eps^2} + \nreset^3 \nmc \frac{AH^2}{\eps^2} + \nreset^2 \nmc \frac{A^2H^2}{\eps^2} \\
     &= \poly \prn*{ \cpush, S, A, H, \log \abs{\Pi}, \frac{1}{\eps}, \log \frac{1}{\delta} } \quad \text{samples.}
\end{align*}
Afterwards, we can rescale $\eps \gets \eps/\wt{O}(SAH^2)$ so that the bound Eq.~\eqref{eq:final-bound} is at most $\eps$, and rescale $\delta \gets \delta / (3 T_\mathsf{D} + T_\mathsf{R} + 1)$ so that the guarantee occurs with probability at least $1-\delta$. The final sample complexity is
\begin{align*}
    \text{\glcomment{TODO}}.
\end{align*}\qed


\clearpage
\subsection{Concentrability Analysis}

\begin{proof}[Proof Attempt]
\glcomment{basically we should check all of the statements which depend on the projection as those only hold of $s$ is $\eps$-reachable itself. modify definiton of $\nrch$ to be those which are $\eps$-reachable from the input state.}
The proof of Part (1) should be similar to what has already been done. We focus on Part (2).

\begin{align*}
    \hspace{2em}&\hspace{-2em} \max_{\pi \in \Pi} \sum_{s \in \latentsp_{h-1}} d^\pi_{h-1}(s) \cdot \err(s)  = \max_{\pi \in \Pi} \sum_{s \in \latentsp_{h-1}} d^\pi_{h-1}(s) \cdot \crl*{ \max_{x \in \estmdpobsspace{h}: \optdec(x) = s} \max_{\pi' \in \Pi}~\abs*{V^{\pi'}(x) - \wh{V}^{\pi'}(x)} }.
\end{align*}
Fix any $(x, \pi)$. We have the following decomposition:
\begin{align*}
\hspace{2em}&\hspace{-2em} \abs*{V^{\pi}(x) - \wh{V}^{\pi}(x)} \\
&=\abs*{Q^{\pi}(x,\pi) - \wh{R}(x, \pi) - \En_{\empobs_h \sim \bar{p}} \wh{V}^\pi(\empobs_h)} \\
&\le \eps + \underbrace{ \abs*{ \En_{s_{h} \sim \samplelatp} V^\pi(s_{h}) - \En_{\empobs_{h} \sim \projR(\samplelatp)} V^\pi(\empobs_{h}) } }_{ \eqqcolon \mathtt{Term}_1} + \underbrace{ \abs*{ \En_{\empobs_{h} \sim \projR(\samplelatp)} V^\pi(\empobs_{h}) - \En_{\empobs_{h} \sim \projR(\samplelatp)} \wh{V}^\pi(\empobs_{h})} }_{\eqqcolon \mathtt{Term}_2} \\
    &\quad\quad + \underbrace{ \abs*{\En_{\empobs_{h} \sim \projR(\samplelatp)} \wh{V}^\pi(\empobs_{h}) - \En_{\empobs_{h} \sim \bar{p}} \wh{V}^\pi(\empobs_{h}) } }_{\eqqcolon \mathtt{Term}_3}
\end{align*}
For $\mathtt{Term}_1$:
\begin{align*}
    \mathtt{Term}_1 &= \abs*{ \En_{s_{h} \sim \samplelatp} V^\pi(s_{h}) - \En_{\empobs_{h} \sim \projR(\samplelatp)} V^\pi(\empobs_{h}) } \\
    &\le \sum_{s_h \in \supp(\projR)^c} \samplelatp(s_h) + \sum_{s_h \in \supp(\projR)} \samplelatp(s_h)~\abs*{V^\pi(s_{h}) - \En_{\empobs_{h} \sim \unif(\cdots)} V^\pi(\empobs_{h})} \\
    &\lesssim S\eps + \sum_{s_h \in \supp(\projR)} \samplelatp(s_h)~\abs*{V^\pi(s_{h}) - \En_{\empobs_{h} \sim \unif(\cdots)} V^\pi(\empobs_{h})}.
\end{align*}
The second inequality follows because $\projR$ is supported on $\crl{s \in \latentsp_h: \optlatp(s) \ge \eps}$. Now we break up the calculation into two cases. Suppose that $s_{h-1}$ is $\eps$-reachable. Then this implies that $s_h$ is $\eps^2$ reachable, so therefore those $s_h$ are well-represented in layer $h$ and the last term can be bounded by $S\eps$. For $s_{h-1}$ which are not $\eps$-reachable then the sum is bounded by $S\eps$ when multiplied by $d^\pi_{h-1}(s)$, so therefore we have shown that
\begin{align*}
    \max_{\pi \in \Pi} \sum_{s \in \latentsp_{h-1}} d^\pi_{h-1}(s) \cdot \mathtt{Term}_1 \le S \eps.
\end{align*}
Now we move onto showing a bound on $\mathtt{Term}_2$.
\begin{align*}
    \max_{\pi \in \Pi} \sum_{s \in \latentsp_{h-1}} d^\pi_{h-1}(s) \cdot \mathtt{Term}_2 &\le \max_{\pi \in \Pi} \sum_{s \in \latentsp_{h-1}} d^\pi_{h-1}(s) \cdot \sum_{s' \in \latentsp_h} \samplelatp(s'|s,\pi) \cdot \err(s')  \\
    &\le \max_{\pi \in \Pi} \sum_{s' \in \latentsp_{h}} \err(s') \sum_{s \in \latentsp_{h-1}} d^\pi_{h-1}(s) \cdot \samplelatp(s'|s,\pi) \\
    &\le \eps + \max_{\pi \in \Pi} \sum_{s' \in \latentsp_{h}} d^\pi_{h}(s') \cdot \err(s') \\
    &\le \eps + \Gamma_h.
\end{align*}
For $\mathtt{Term}_3$:
\begin{align*}
    \max_{\pi \in \Pi} \sum_{s \in \latentsp_{h-1}} d^\pi_{h-1}(s) \cdot \mathtt{Term}_3 \coloneqq \max_{\pi \in \Pi} \sum_{s \in \latentsp_{h-1}} d^\pi_{h-1}(s) \cdot  \abs*{\En_{\empobs_{h} \sim \projR(\samplelatp)} \wh{V}^\pi(\empobs_{h}) - \En_{\empobs_{h} \sim \bar{p}} \wh{V}^\pi(\empobs_{h}) }
\end{align*}
Again, we only need to control this term for the $s$ which are $\eps$-reachable at layer $h-1$. The last term only depends on the sampling at layer $h$?
\end{proof}

\subsection{Some Older Lemmas}
Let us define $\epsRS{h} \coloneqq \crl{s \in \latentsp_h: \max_{\pi \in \Pi} d^\pi_h(s) \ge \eps}$.

\begin{proposition}
Let $(s,a) \in \epsRS{h} \times \actionsp$.Then if $s' \in  \crl{s \in \latentsp: \optlatp(s' ~|~ s, a) \ge \eps/S}$, we know that $s'$ is $\eps^2/S$-reachable.
\end{proposition}

\begin{proposition}
Suppose $\mu$ satisfies \pref{ass:exploratory-conc-distribution}. Then for any $s' \in \epsRS{h}$,
\begin{align*}
    \max_{s,a} \frac{\optlatp(s'~|~s,a)}{\mu_h(s')} \le \frac{\cpi S}{\eps}.
\end{align*}
\end{proposition}
\begin{proof}
Fix any $s' \in \cS_{h}$, and let $\wt{\pi} = \argmax_{\pi \in \Pi} d^{\pi}_{h}(s')$. Observe that there must exist some $s \in \cS_{h-1}$ such that $d^{\wt{\pi}}(s) \ge \eps/S$, since
\begin{align*}
    \eps \le d^{\wt{\pi}}_{h}(s') = \sum_{s} \optlatp(s'|s, \wt{\pi}) \cdot d^{\wt{\pi}}_{h-1}(s).
\end{align*}
Then we have
\begin{align*}
    \max_{s,a} \frac{\optlatp(s'|s,a)}{\mu_h(s')} = \max_{s,a} \frac{\optlatp(s'|s,a)}{\mu_h(s')} \cdot \frac{d^{\wt{\pi}}(s)}{d^{\wt{\pi}}(s)} \le \max_{s,a} \frac{d^{\wt{\pi} \circ a}(s')}{\mu_h(s')} \cdot  \frac{1}{d^{\wt{\pi}}(s)} \le \cpi \cdot \max_{s} \frac{1}{d^{\wt{\pi}}(s)} \le \frac{\cpi S}{\eps}.
\end{align*}
\end{proof}


\glcomment{
\begin{itemize}
    \item \stochrefit{} analysis: We can just cap the number of gradient updates for every $(x,a)$, and thus bound the total sample complexity.
\end{itemize} Summary of ideas to make for the concentrability setting.
- proj_1 is the projection on the eps-pushforward reachable states from (s,a).
- proj_2 is the projection onto states which are both eps-pushforward and eps-globally reachable states.
- construct confidence sets using proj_1.
- for refitting:
    - if state has been updated many times, then replace it with a terminal state.
    - potential function to track is regret against proj_2. 
    - however since we project to P, proj_2 may not be in P. However this incurs some additive misspeicification so the total number of refits can be bounded per state.
}


